Optimal Primal-Dual Algorithm with Last iterate Convergence Guarantees for Stochastic Convex Optimization Problems

This paper proposes a novel first-order algorithm that solves composite nonsmooth and stochastic convex optimization problem with function constraints. Most of the works in the literature provide convergence rate guarantees on the average-iterate solution. There is growing interest in the convergence guarantees of the last iterate solution due to its favorable structural properties, such as sparsity or privacy guarantees and good performance in practice. We provide the first method that obtains the best-known convergence rate guarantees on the last iterate for stochastic composite nonsmooth convex function-constrained optimization problems. Our novel and easy-to-implement algorithm is based on the augmented Lagrangian technique and uses a new linearized approximation of constraint functions, leading to its name, the Augmented Constraint Extrapolation (Aug-ConEx) method. We show that Aug-ConEx achieves $\mathcal{O}(1/\sqrt{K})$ convergence rate in the nonsmooth stochastic setting without any strong convexity assumption and $\mathcal{O}(1/K)$ for the same problem with strongly convex objective function. While optimal for nonsmooth and stochastic problems, the Aug-ConEx method also accelerates convergence in terms of Lipschitz smoothness constants to $\mathcal{O}(1/K)$ and $\mathcal{O}(1/K^2)$ in the aforementioned cases, respectively. To our best knowledge, this is the first method to obtain such differentiated convergence rate guarantees on the last iterate for a composite nonsmooth stochastic setting without additional $\log{K}$ factors. We validate the efficiency of our algorithm by comparing it with a state-of-the-art algorithm through numerical experiments.

==> ref.tex <==
@article{liang2024unified,
  title={A unified analysis of a class of proximal bundle methods for solving hybrid convex composite optimization problems},
  author={Liang, Jiaming and Monteiro, Renato DC},
  journal={Mathematics of Operations Research},
  volume={49},
  number={2},
  pages={832--855},
  year={2024},
  publisher={INFORMS}
}

@article{cai2024last,
  title={Last iterate convergence of incremental methods and applications in continual learning},
  author={Cai, Xufeng and Diakonikolas, Jelena},
  journal={arXiv preprint arXiv:2403.06873},
  year={2024}
}

@article{polyak1992acceleration,
  title={Acceleration of stochastic approximation by averaging},
  author={Polyak, Boris T and Juditsky, Anatoli B},
  journal={SIAM journal on control and optimization},
  volume={30},
  number={4},
  pages={838--855},
  year={1992},
  publisher={SIAM}
}


@inproceedings{zinkevich2003online,
  title={Online convex programming and generalized infinitesimal gradient ascent},
  author={Zinkevich, Martin},
  booktitle={Proceedings of the 20th international conference on machine learning (icml-03)},
  pages={928--936},
  year={2003}
}

@article{rakhlin2011making,
  title={Making gradient descent optimal for strongly convex stochastic optimization},
  author={Rakhlin, Alexander and Shamir, Ohad and Sridharan, Karthik},
  journal={arXiv preprint arXiv:1109.5647},
  year={2011}
}

@article{deng2018optimal,
  title={Optimal adaptive and accelerated stochastic gradient descent},
  author={Deng, Qi and Cheng, Yi and Lan, Guanghui},
  journal={arXiv preprint arXiv:1810.00553},
  year={2018}
}

@inproceedings{yu2016primal,
  title={A primal-dual type algorithm with the O (1/t) convergence rate for large scale constrained convex programs},
  author={Yu, Hao and Neely, Michael J},
  booktitle={2016 IEEE 55th Conference on Decision and Control (CDC)},
  pages={1900--1905},
  year={2016},
  organization={IEEE}
}

@article{cartis2011evaluation,
  title={On the evaluation complexity of composite function minimization with applications to nonconvex nonlinear programming},
  author={Cartis, Coralia and Gould, Nicholas IM and Toint, Philippe L},
  journal={SIAM Journal on Optimization},
  volume={21},
  number={4},
  pages={1721--1739},
  year={2011},
  publisher={SIAM}
}

@article{kong2019complexity,
  title={Complexity of a quadratic penalty accelerated inexact proximal point method for solving linearly constrained nonconvex composite programs},
  author={Kong, Weiwei and Melo, Jefferson G and Monteiro, Renato DC},
  journal={SIAM Journal on Optimization},
  volume={29},
  number={4},
  pages={2566--2593},
  year={2019},
  publisher={SIAM}
}

@article{li2021augmented,
  title={Augmented Lagrangian--based first-order methods for convex-constrained programs with weakly convex objective},
  author={Li, Zichong and Xu, Yangyang},
  journal={INFORMS Journal on Optimization},
  volume={3},
  number={4},
  pages={373--397},
  year={2021},
  publisher={INFORMS}
}

@article{lin2022complexity,
  title={Complexity of an inexact proximal-point penalty method for constrained smooth non-convex optimization},
  author={Lin, Qihang and Ma, Runchao and Xu, Yangyang},
  journal={Computational optimization and applications},
  volume={82},
  number={1},
  pages={175--224},
  year={2022},
  publisher={Springer}
}

@article{lan2013iteration,
  title={Iteration-complexity of first-order penalty methods for convex programming},
  author={Lan, Guanghui and Monteiro, Renato DC},
  journal={Mathematical Programming},
  volume={138},
  number={1},
  pages={115--139},
  year={2013},
  publisher={Springer}
}

@article{lan2016iteration,
  title={Iteration-complexity of first-order augmented Lagrangian methods for convex programming},
  author={Lan, Guanghui and Monteiro, Renato DC},
  journal={Mathematical Programming},
  volume={155},
  number={1},
  pages={511--547},
  year={2016},
  publisher={Springer}
}

@article{xu2021iteration,
  title={Iteration complexity of inexact augmented Lagrangian methods for constrained convex programming},
  author={Xu, Yangyang},
  journal={Mathematical Programming},
  volume={185},
  pages={199--244},
  year={2021},
  publisher={Springer}
}

@article{xu2020primal,
  title={Primal-dual stochastic gradient method for convex programs with many functional constraints},
  author={Xu, Yangyang},
  journal={SIAM Journal on Optimization},
  volume={30},
  number={2},
  pages={1664--1692},
  year={2020},
  publisher={SIAM}
}

@article{xu2022first,
  title={First-order methods for problems with O (1) functional constraints can have almost the same convergence rate as for unconstrained problems},
  author={Xu, Yangyang},
  journal={SIAM Journal on Optimization},
  volume={32},
  number={3},
  pages={1759--1790},
  year={2022},
  publisher={SIAM}
}

@article{li2021inexact,
  title={An inexact proximal augmented Lagrangian framework with arbitrary linearly convergent inner solver for composite convex optimization},
  author={Li, Fei and Qu, Zheng},
  journal={Mathematical Programming Computation},
  volume={13},
  pages={583--644},
  year={2021},
  publisher={Springer}
}

@article{nedic2009approximate,
  title={Approximate primal solutions and rate analysis for dual subgradient methods},
  author={Nedi{\'c}, Angelia and Ozdaglar, Asuman},
  journal={SIAM Journal on Optimization},
  volume={19},
  number={4},
  pages={1757--1780},
  year={2009},
  publisher={SIAM}
}

@article{Pol67,
    author = {B.~T.~Polyak},
    title = {A general method for solving extremal problems},
    journal = {Dokl. Akad. Nauk SSSR},
    year = {1967},
    volume = {174},
    number = {1},
    pages = {33--36}
}

@article{nesterov83,
    author = {Y.~Nesterov},
    title = {A method of solving a convex programming problem with convergence rate O(1/k2)},
    journal = {Dokl. Akad. Nauk SSSR},
    year = {1983},
    volume = {27},
    number = {2},
    pages = {372--376}
}

@article{solodov2007explicit,
  title={An explicit descent method for bilevel convex optimization},
  author={Solodov, Mikhail},
  journal={Journal of Convex Analysis},
  volume={14},
  number={2},
  pages={227},
  year={2007},
  publisher={HELDERMANN VERLAG LANGER GRABEN 17, 32657 LEMGO, GERMANY}
}

@article{samadi2023improved,
  title={Improved guarantees for optimal Nash equilibrium seeking and bilevel variational inequalities},
  author={Samadi, Sepideh and Yousefian, Farzad},
  journal={arXiv preprint arXiv:2307.12511},
  year={2023}
}

@article{helou2017e,
  title={e-subgradient algorithms for bilevel convex optimization},
  author={Helou, Elias S and Sim{\~o}es, Lucas EA},
  journal={Inverse problems},
  volume={33},
  number={5},
  pages={055020},
  year={2017},
  publisher={IOP Publishing}
}

@article{kaushik2021method,
  title={A method with convergence rates for optimization problems with variational inequality constraints},
  author={Kaushik, Harshal D and Yousefian, Farzad},
  journal={SIAM Journal on Optimization},
  volume={31},
  number={3},
  pages={2171--2198},
  year={2021},
  publisher={SIAM}
}

@article{lemarechal1995new,
  title={New variants of bundle methods},
  author={Lemar{\'e}chal, Claude and Nemirovskii, Arkadii and Nesterov, Yurii},
  journal={Mathematical programming},
  volume={69},
  pages={111--147},
  year={1995},
  publisher={Springer}
}

@book{nesterov2018lectures,
  title={Lectures on convex optimization},
  author={Nesterov, Yurii and others},
  volume={137},
  year={2018},
  publisher={Springer}
}

@book{nemirovskij1983problem,
  title={Problem complexity and method efficiency in optimization},
  author={Nemirovskij, Arkadij Semenovi{\v{c}} and Yudin, David Borisovich},
  year={1983},
  publisher={Wiley-Interscience}
}
@article{lin2018level,
  title={A level-set method for convex optimization with a feasible solution path},
  author={Lin, Qihang and Nadarajah, Selvaprabu and Soheili, Negar},
  journal={SIAM Journal on Optimization},
  volume={28},
  number={4},
  pages={3290--3311},
  year={2018},
  publisher={SIAM}
}

@article{chambolle2011first,
  title={A first-order primal-dual algorithm for convex problems with applications to imaging},
  author={Chambolle, Antonin and Pock, Thomas},
  journal={Journal of mathematical imaging and vision},
  volume={40},
  pages={120--145},
  year={2011},
  publisher={Springer}
}

@article{chambolle2016ergodic,
  title={On the ergodic convergence rates of a first-order primal--dual algorithm},
  author={Chambolle, Antonin and Pock, Thomas},
  journal={Mathematical Programming},
  volume={159},
  number={1},
  pages={253--287},
  year={2016},
  publisher={Springer}
}

@article{chen2014optimal,
  title={Optimal primal-dual methods for a class of saddle point problems},
  author={Chen, Yunmei and Lan, Guanghui and Ouyang, Yuyuan},
  journal={SIAM Journal on Optimization},
  volume={24},
  number={4},
  pages={1779--1814},
  year={2014},
  publisher={SIAM}
}

@inproceedings{thekumparampil2022lifted,
  title={Lifted primal-dual method for bilinearly coupled smooth minimax optimization},
  author={Thekumparampil, Kiran K and He, Niao and Oh, Sewoong},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={4281--4308},
  year={2022},
  organization={PMLR}
}

@article{hamedani2021primal,
  title={A primal-dual algorithm with line search for general convex-concave saddle point problems},
  author={Hamedani, Erfan Yazdandoost and Aybat, Necdet Serhat},
  journal={SIAM Journal on Optimization},
  volume={31},
  number={2},
  pages={1299--1329},
  year={2021},
  publisher={SIAM}
}

@inproceedings{khalafi2023accelerated,
  title={Accelerated primal-dual methods for convex-strongly-concave saddle point problems},
  author={Khalafi, Mohammad and Boob, Digvijay},
  booktitle={International Conference on Machine Learning},
  pages={16250--16270},
  year={2023},
  organization={PMLR}
}

@inproceedings{shamir2013stochastic,
  title={Stochastic gradient descent for non-smooth optimization: Convergence results and optimal averaging schemes},
  author={Shamir, Ohad and Zhang, Tong},
  booktitle={International conference on machine learning},
  pages={71--79},
  year={2013},
  organization={PMLR}
}

@inproceedings{harvey2019tight,
  title={Tight analyses for non-smooth stochastic gradient descent},
  author={Harvey, Nicholas JA and Liaw, Christopher and Plan, Yaniv and Randhawa, Sikander},
  booktitle={Conference on Learning Theory},
  pages={1579--1613},
  year={2019},
  organization={PMLR}
}

@article{jain2021making,
  title={Making the last iterate of sgd information theoretically optimal},
  author={Jain, Prateek and Nagaraj, Dheeraj M and Netrapalli, Praneeth},
  journal={SIAM Journal on Optimization},
  volume={31},
  number={2},
  pages={1108--1130},
  year={2021},
  publisher={SIAM}
}

@article{liu2023revisiting,
  title={Revisiting the last-iterate convergence of stochastic gradient methods},
  author={Liu, Zijian and Zhou, Zhengyuan},
  journal={arXiv preprint arXiv:2312.08531},
  year={2023}
}

@article{shamir2012averaging,
  title={Is averaging needed for strongly convex stochastic gradient descent},
  author={Shamir, Ohad},
  journal={Open problem presented at COLT},
  year={2012}
}

@inproceedings{shalev2007pegasos,
  title={Pegasos: Primal estimated sub-gradient solver for svm},
  author={Shalev-Shwartz, Shai and Singer, Yoram and Srebro, Nathan},
  booktitle={Proceedings of the 24th international conference on Machine learning},
  pages={807--814},
  year={2007}
}

@inproceedings{feldman2018privacy,
  title={Privacy amplification by iteration},
  author={Feldman, Vitaly and Mironov, Ilya and Talwar, Kunal and Thakurta, Abhradeep},
  booktitle={2018 IEEE 59th Annual Symposium on Foundations of Computer Science (FOCS)},
  pages={521--532},
  year={2018},
  organization={IEEE}
}

@article{altschuler2022privacy,
  title={Privacy of noisy stochastic gradient descent: More iterations without more privacy loss},
  author={Altschuler, Jason and Talwar, Kunal},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={3788--3800},
  year={2022}
}

@article{asoodeh2023privacy,
  title={Privacy Loss of Noisy Stochastic Gradient Descent Might Converge Even for Non-Convex Losses},
  author={Asoodeh, Shahab and Diaz, Mario},
  journal={arXiv preprint arXiv:2305.09903},
  year={2023}
}

@article{boob2024level,
  title={Level constrained first order methods for function constrained optimization},
  author={Boob, Digvijay and Deng, Qi and Lan, Guanghui},
  journal={Mathematical Programming},
  pages={1--61},
  year={2024},
  publisher={Springer}
}

@Article{Jordan2023,
  author  = {Jordan, Michael I. and Lin, Tianyi and Zampetakis, Manolis},
  journal = {Journal of Machine Learning Research},
  title   = {First-Order Algorithms for Nonlinear Generalized Nash Equilibrium Problems},
  year    = {2023},
  issn    = {1533-7928},
  number  = {38},
  pages   = {1-46},
  volume  = {24},
}

@article{lan2020algorithms,
  title={Algorithms for stochastic optimization with function or expectation constraints},
  author={Lan, Guanghui and Zhou, Zhiqiang},
  journal={Computational Optimization and Applications},
  volume={76},
  number={2},
  pages={461--498},
  year={2020},
  publisher={Springer}
}

@article{aravkin2019level,
  title={Level-set methods for convex optimization},
  author={Aravkin, Aleksandr Y and Burke, James V and Drusvyatskiy, Dmitry and Friedlander, Michael P and Roy, Scott},
  journal={Mathematical Programming},
  volume={174},
  pages={359--390},
  year={2019},
  publisher={Springer}
}

@article{yu2017online,
  title={Online convex optimization with stochastic constraints},
  author={Yu, Hao and Neely, Michael and Wei, Xiaohan},
  journal={Advances in Neural Information Processing Systems},
  volume={30},
  year={2017}
}

@article{huang2022new,
  title={New first-order algorithms for stochastic variational inequalities},
  author={Huang, Kevin and Zhang, Shuzhong},
  journal={SIAM Journal on Optimization},
  volume={32},
  number={4},
  pages={2745--2772},
  year={2022},
  publisher={SIAM}
}
@Article{Chavdarova2022,
  author  = {Chavdarova, Tatjana and Pagliardini, Matteo and Yang, Tong and Jordan, Michael I.},
  journal = {arXiv preprint arXiv:2210.15659},
  title   = {Revisiting the ACVI Method for Constrained Variational Inequalities},
  year    = {2022},
  groups  = {VI},
}

@article{boob2021optimal,
  title={Optimal algorithms for differentially private stochastic monotone variational inequalities and saddle-point problems},
  author={Boob, Digvijay and Guzm{\'a}n, Crist{\'o}bal},
  journal={arXiv preprint arXiv:2104.02988},
  year={2021},
  groups  = {VI},
}

@article{boob2023stochastic,
  title={Stochastic first-order methods for convex and nonconvex functional constrained optimization},
  author={Boob, Digvijay and Deng, Qi and Lan, Guanghui},
  journal={Mathematical Programming},
  volume={197},
  number={1},
  pages={215--279},
  year={2023},
  publisher={Springer}
}

@book{facchinei2003finite,
  title={Finite-dimensional variational inequalities and complementarity problems},
  author={Facchinei, Francisco and Pang, Jong-Shi},
  year={2003},
  publisher={Springer}
}

@Article{Yang2022Solving,
  author  = {Yang, Tong and Jordan, Michael I. and Chavdarova, Tatjana},
  journal = {arXiv preprint arXiv:2206.10575},
  title   = {Solving constrained variational inequalities via an interior point method},
  year    = {2022},
  groups  = {VI},
}

@Article{Dai2022,
  author  = {Dai, Yu-Hong and Zhang, Li-Wei},
  journal = {Journal of the Operations Research Society of China},
  title   = {The Rate of Convergence of Augmented Lagrangian Method for Minimax Optimization Problems with Equality Constraints},
  year    = {2022},
  issn    = {2194-668X},
  pages   = {1-33},
  groups  = {VI},
  type    = {Journal Article},
}

@inproceedings{alacaoglu2022stochastic,
  title={Stochastic variance reduction for variational inequality methods},
  author={Alacaoglu, Ahmet and Malitsky, Yura},
  booktitle={Conference on Learning Theory},
  pages={778--816},
  year={2022},
  organization={PMLR}
}

@Article{Kotsalis2022,
  author  = {Kotsalis, Georgios and Lan, Guanghui and Li, Tianjiao},
  journal = {SIAM Journal on Optimization},
  title   = {Simple and optimal methods for stochastic variational inequalities, I: Operator extrapolation},
  year    = {2022},
  issn    = {1052-6234},
  number  = {3},
  pages   = {2041-2073},
  volume  = {32},
  groups  = {VI},
}


@article{mokhtari2020convergence,
  title={Convergence rate of O(1/k) for optimistic gradient and extragradient methods in smooth convex-concave saddle point problems},
  author={Mokhtari, Aryan and Ozdaglar, Asuman E and Pattathil, Sarath},
  journal={SIAM Journal on Optimization},
  volume={30},
  number={4},
  pages={3230--3251},
  year={2020},
  publisher={SIAM}
}


@article{goodfellow2020generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Communications of the ACM},
  volume={63},
  number={11},
  pages={139--144},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@Article{Dai2020,
  author  = {Dai, Yu-Hong and Zhang, Liwei},
  journal = {arXiv preprint arXiv:2004.09730},
  title   = {Optimality conditions for constrained minimax optimization},
  year    = {2020},
  type    = {Journal Article},
}

@Article{Dai2022a,
  author  = {Dai, Yu-Hong and Wang, Jiani and Zhang, Liwei},
  journal = {arXiv preprint arXiv:2204.09185},
  title   = {Optimality conditions and numerical algorithms for a class of linearly constrained minimax optimization problems},
  year    = {2022},
  type    = {Journal Article},
}

@Article{Lu2023,
  author  = {Lu, Zhaosong and Mei, Sanyou},
  journal = {arXiv preprint arXiv:2301.02060},
  title   = {A first-order augmented Lagrangian method for constrained minimax optimization},
  year    = {2023},
  groups  = {VI},
  type    = {Journal Article},
}

@Article{Tsaknakis2021,
  author  = {Tsaknakis, Ioannis and Hong, Mingyi and Zhang, Shuzhong},
  journal = {arXiv preprint arXiv:2110.11210},
  title   = {Minimax problems with coupled linear constraints: computational complexity, duality and solution methods},
  year    = {2021},
  type    = {Journal Article},
}

@Article{Yang2022a,
  author  = {Yang, Shuoguang and Li, Xudong and Lan, Guanghui},
  journal = {arXiv preprint arXiv:2202.07868},
  title   = {Data-Driven Minimax Optimization with Expectation Constraints},
  year    = {2022},
  groups  = {VI},
}

@inproceedings{GidelBVVL19,
  author    = {Gauthier Gidel and
               Hugo Berard and
               Ga{\"{e}}tan Vignoud and
               Pascal Vincent and
               Simon Lacoste{-}Julien},
  title     = {A Variational Inequality Perspective on Generative Adversarial Networks},
  booktitle = {7th International Conference on Learning Representations, {ICLR}},
  year      = {2019}
}

@article{yousefian2017smoothing,
  title={On smoothing, regularization, and averaging in stochastic approximation methods for stochastic variational inequality problems},
  author={Yousefian, Farzad and Nedi{\'c}, Angelia and Shanbhag, Uday V},
  journal={Mathematical Programming},
  volume={165},
  pages={391--431},
  year={2017},
  publisher={Springer}
}

@article{malitsky2015projected,
  title={Projected reflected gradient methods for monotone variational inequalities},
  author={Malitsky, Yu},
  journal={SIAM Journal on Optimization},
  volume={25},
  number={1},
  pages={502--520},
  year={2015},
  publisher={SIAM}
}

@article{auslender2010moving,
  title={A moving balls approximation method for a class of smooth constrained minimization problems},
  author={Auslender, Alfred and Shefi, Ron and Teboulle, Marc},
  journal={SIAM Journal on Optimization},
  volume={20},
  number={6},
  pages={3232--3259},
  year={2010},
  publisher={SIAM}
}

@article{auslender2013very,
  title={A very simple SQCQP method for a class of smooth convex constrained minimization problems with nice convergence results},
  author={Auslender, Alfred},
  journal={Mathematical Programming},
  volume={142},
  pages={349--369},
  year={2013},
  publisher={Springer}
}

@article{singh2024stochastic,
  title={A stochastic moving ball approximation method for smooth convex constrained minimization},
  author={Singh, Nitesh Kumar and Necoara, Ion},
  journal={Computational Optimization and Applications},
  pages={1--31},
  year={2024},
  publisher={Springer}
}

@article{zhu2022new,
  title={New primal-dual algorithms for a class of nonsmooth and nonlinear convex-concave minimax problems},
  author={Zhu, Yuzixuan and Liu, Deyi and Tran-Dinh, Quoc},
  journal={SIAM Journal on Optimization},
  volume={32},
  number={4},
  pages={2580--2611},
  year={2022},
  publisher={SIAM}
}

@article{zhang2022solving,
  title={Solving Convex Smooth Function Constrained Optimization Is Almost As Easy As Unconstrained Optimization},
  author={Zhang, Zhe and Lan, Guanghui},
  journal={arXiv preprint arXiv:2210.05807},
  year={2022}
}

@inproceedings{yousefian2014optimal,
  title={Optimal robust smoothing extragradient algorithms for stochastic variational inequality problems},
  author={Yousefian, Farzad and Nedi{\'c}, Angelia and Shanbhag, Uday V},
  booktitle={53rd IEEE conference on decision and control},
  pages={5831--5836},
  year={2014},
  organization={IEEE}
}

@incollection{shanbhag2013stochastic,
  title={Stochastic variational inequality problems: Applications, analysis, and algorithms},
  author={Shanbhag, Uday V},
  booktitle={Theory driven by influential applications},
  pages={71--107},
  year={2013},
  publisher={INFORMS}
}

@article{koshal2012regularized,
  title={Regularized iterative stochastic approximation methods for stochastic variational inequality problems},
  author={Koshal, Jayash and Nedic, Angelia and Shanbhag, Uday V},
  journal={IEEE Transactions on Automatic Control},
  volume={58},
  number={3},
  pages={594--609},
  year={2012},
  publisher={IEEE}
}

@article{juditsky2011solving,
  title={Solving variational inequalities with stochastic mirror-prox algorithm},
  author={Juditsky, Anatoli and Nemirovski, Arkadi and Tauvel, Claire},
  journal={Stochastic Systems},
  volume={1},
  number={1},
  pages={17--58},
  year={2011},
  publisher={INFORMS}
}

@article{bertsekas2011approximate,
  title={Approximate policy iteration: A survey and some new methods},
  author={Bertsekas, Dimitri P},
  journal={Journal of Control Theory and Applications},
  volume={9},
  number={3},
  pages={310--335},
  year={2011},
  publisher={Springer}
}

@article{pang1982iterative,
	title={Iterative methods for variational and complementarity problems},
	author={Pang, Jong-Shi and Chan, Donald},
	journal={Mathematical programming},
	volume={24},
	number={1},
	pages={284--313},
	year={1982},
	publisher={Springer}
}

@techreport{josephy1979newton,
	title={Newton's Method for Generalized Equations.},
	author={Josephy, Norman H},
	number = {1965},
	year={1979},
	institution = {Wisconsin Univ-Madison Mathematics Research Center},
}

@techreport{josephy1979quasi,
	title={Quasi-Newton methods for generalized equations},
	author={Josephy, Norman H},
	number = {1966},
	year={1979},
	institution={Wisconsin Univ-Madison Mathematics Research Center}
}
@techreport{subramanian1985gauss,
	title={Gauss-Newton Methods for the Nonlinear Complementarity Problem.},
	author={Subramanian, PK},
	number = {2845},
	year={1985},
	institution={Wisconsin Univ-Madison Mathematics Research Center}
}

@article{ben2002robust,
  title={Robust optimization--methodology and applications},
  author={Ben-Tal, Aharon and Nemirovski, Arkadi},
  journal={Mathematical programming},
  volume={92},
  pages={453--480},
  year={2002},
  publisher={Springer}
}

@article{ralph2000superlinear,
  title={Superlinear convergence of an interior-point method despite dependent constraints},
  author={Ralph, Daniel and Wright, Stephen J},
  journal={Mathematics of Operations Research},
  volume={25},
  number={2},
  pages={179--194},
  year={2000},
  publisher={INFORMS}
}

@article{harker1990finite,
  title={Finite-dimensional variational inequality and nonlinear complementarity problems: a survey of theory, algorithms and applications},
  author={Harker, Patrick T and Pang, Jong-Shi},
  journal={Mathematical programming},
  volume={48},
  number={1-3},
  pages={161--220},
  year={1990},
  publisher={Springer}
}

@article{qi2002smoothing,
  title={Smoothing functions and smoothing Newton method for complementarity and variational inequality problems},
  author={Qi, Liqun and Sun, Defeng and others},
  journal={Journal of Optimization Theory and Applications},
  volume={113},
  number={1},
  pages={121--147},
  year={2002},
  publisher={Kluwer Academic/Plenum Publishers}
}

@book{mangasarian1994nonlinear,
  title={Nonlinear programming},
  author={Mangasarian, Olvi L},
  year={1994},
  publisher={SIAM}
}

@book{bertsekas99nonlinear,
  author = {Bertsekas, D.P.},
  publisher = {Athena Scientific},
  title = {Nonlinear Programming},
  year = {1999}
}

@article{nesterov2011solving,
  title={Solving strongly monotone variational and quasi-variational inequalities},
  author={Nesterov, Yurii and Scrimali, Laura},
  journal={Discrete and Continuous Dynamical Systems},
  volume={31},
  number={4},
  pages={1383--1396},
  year={2011},
  publisher={Discrete and Continuous Dynamical Systems}
}

@article{pang2010design,
  title={Design of cognitive radio systems under temperature-interference constraints: A variational inequality approach},
  author={Pang, Jong-Shi and Scutari, Gesualdo and Palomar, Daniel P and Facchinei, Francisco},
  journal={IEEE Transactions on Signal Processing},
  volume={58},
  number={6},
  pages={3251--3271},
  year={2010},
  publisher={IEEE}
}

@article{facchinei2007generalized,
  title={On generalized Nash games and variational inequalities},
  author={Facchinei, Francisco and Fischer, Andreas and Piccialli, Veronica},
  journal={Operations Research Letters},
  volume={35},
  number={2},
  pages={159--164},
  year={2007},
  publisher={Elsevier}
}


@article{jiang2008stochastic,
  title={Stochastic approximation approaches to the stochastic variational inequality problem},
  author={Jiang, Houyuan and Xu, Huifu},
  journal={IEEE Transactions on Automatic Control},
  volume={53},
  number={6},
  pages={1462--1475},
  year={2008},
  publisher={IEEE}
}



@Article{Nesterov2007,
  author    = {Nesterov, Yurii},
  journal   = {Mathematical Programming},
  title     = {Dual extrapolation and its applications to solving variational inequalities and related problems},
  year      = {2007},
  number    = {2-3},
  pages     = {319--344},
  volume    = {109},
  groups    = {VI},
  publisher = {Springer},
}

@Article{Nemirovski2004,
  author    = {Nemirovski, Arkadi},
  journal   = {SIAM Journal on Optimization},
  title     = {Prox-method with rate of convergence O (1/t) for variational inequalities with Lipschitz continuous monotone operators and smooth convex-concave saddle point problems},
  year      = {2004},
  number    = {1},
  pages     = {229--251},
  volume    = {15},
  groups    = {VI},
  publisher = {SIAM},
}

@article{popov1980modification,
  title={A modification of the Arrow-Hurwicz method for search of saddle points},
  author={Popov, Leonid Denisovich},
  journal={Mathematical notes of the Academy of Sciences of the USSR},
  volume={28},
  pages={845--848},
  year={1980},
  publisher={Springer}
}

@Article{Korpelevich1976,
  author  = {Korpelevich, Galina M},
  journal = {Matecon},
  title   = {The extragradient method for finding saddle points and other problems},
  year    = {1976},
  pages   = {747--756},
  volume  = {12},
  groups  = {VI},
}

@article{robbins1951stochastic,
  title={A stochastic approximation method},
  author={Robbins, Herbert and Monro, Sutton},
  journal={The annals of mathematical statistics},
  pages={400--407},
  year={1951},
  publisher={JSTOR}
}

==> sec-convergence-analysis.tex <==
\section{Convergence Analysis of $ \augconex $ Method } \label{sec:convegence-analysis-augconex}
In this section, we provide a comprehensive analysis of Theorem \ref{thm:non-ergo-strong-semi} and Theorem \ref{thm:convex-case}. First, since $\augconex$ is a primal-dual algorithm, one can use the primal-dual gap as a measure of convergence. In particular, for two feasible solutions $z = (x,s,y)$ and $\bar{z} = (\bar{x},\bar{s},\bar{y})$, one can define the primal-dual gap as follows 
\[
Gap:= \Lcal(\bar{x},\bar{s},y) - \Lcal(x,s,\bar{y}).
\]
In the following key lemma, we construct a recursive relation in terms of the iterates $\{x_{k+1},s_{k+1},\tilde{y}_{k+1},\bar{y}_{k+1}\}_{k\geq 1}$ generated by Algorithm \ref{alg:augConEx}. Before formally stating the lemma,
   notice from optimality of $s_{k+1}$ and the definition of $y_{k+1}$ based on \eqref{eq:Denotes} of Algorithm \ref{alg:augConEx}, one can say $y_{k+1}= -\grad h(s_{k+1})$ where
\[
h(s): = \inprod{-\wt{y}_k}{s} + \tfrac{\rho_k}{2}\gnorm{\ell_g(x_{k+1})+ \chi(x_{k+1}) - (1-\tau_k)V_k -s}{}{2}.
\]
Moreover, since $\grad h(s_{k+1})  + N_{\{s:s\leq \mathbf{0}\}}(s_{k+1})\ni \mathbf{0} $, one can conclude that $y_{k+1}\in  N_{\{s:s\leq \mathbf{0}\}}(s_{k+1})$ meaning $y_{k+1}\geq \mathbf{0}$. Now, we are ready to mention the Lemma \ref{lemma:importantlemma}. 
\begin{lemma}\label{lemma:importantlemma}
	Suppose $\tfrac{\eta_k}{2} \le \rho_k$ and $L_k\geq 2L_f+2BL_g$, where $B\geq 0$. Then for all $(x,s,y)\in X\times \mathbb{R}_{-}^m\times\mathbb{R}_{+}^m$ and $k=1,\dots, K-1$, we have
	\begin{align*}
		\Lcal(x_{k+1}, &s_{k+1}, y) - \Lcal(x,s,\wb{y}_{k+1}) - (1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)] \\
		&\le\tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2} -\tau_k\inner{\delta_k }{\dot{x}_k-x} \nonumber\\
		&\quad + \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} ] + \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}- \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2.  
	\end{align*}
	where $\ell_g(x_{k+1}) $ is defined as \eqref{eq:ell_g}, $\delta_k = f'(\hat{x}_k) - \mathfrak{F}(\hat{x}_k,\xi_k)$ and $\dot{x}_k = \tfrac{\hat{x}_k-(1-\tau_{k})x_k}{\tau_k}$. 
\end{lemma}
\begin{proof}
	First, using optimality of $x_{k+1}$, we have for all $x\in X$
	\begin{equation}\label{eq:int_rel2}
		\begin{aligned}
			\inprod{f'(\wh{x}_k) + g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x}&+ \inner{\delta_k }{\hat{x}_k-x} + \chi_0(x_{k+1}) - \chi_0(x) + \inner{\chi(x_{k+1})-\chi(x))}{y_{k+1}} \\
			& \le \tfrac{L_k}{2} [\gnorm{x-\wh{x}_k}{}{2} - \gnorm{x-x_{k+1}}{}{2} - \gnorm{x_{k+1}-\wh{x}_k}{}{2}]+\inner{\delta_k}{\hat{x}_k-x_{k+1}}.
		\end{aligned}
	\end{equation}
	Using strong-convexity and convexity of $f, g$ respectively, Lipschitz property of $f$ and definition of $\ell_g(x_{k+1})$, we have for all $x\in X$
	\begin{align*}
		f(x_{k+1}) &\le f(\wh{x}_k) + \inprod{f'(\wh{x}_k)}{x_{k+1}-\wh{x}_k} + \tfrac{L_f}{2}\gnorm{x_{k+1}-\wh{x}_k}{}{2} + H_f\gnorm{x_{k+1}-\wh{x}_k}{}{},\\
		f(\wh{x}_k) &\le f(x) + \inprod{f'(\wh{x}_k)}{\wh{x}_k-x}- \tfrac{\mu_f\|x-\hat{x}_k\|^2}{2},\\
		g(\wh{x}_k) &\le g(x) + \inprod{g'(\wh{x}_k)}{\wh{x}_k-x},\\
		\ell_g(x_{k+1})&= g(\wh{x}_k) + \inprod{g'(\wh{x}_k)}{x_{k+1}-\wh{x}_k}.
		% \inprod{f'(\wh{x}_k) + g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x}
		% &= \inprod{f'(\wh{x}_k) }{x_{k+1}-\wh{x}_k+ \wh{x}_k - x} + \inprod{g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x} 
		% \ge f(x_{k+1})-f(\wh{x}_k) - \tfrac{L_f}{2}\gnorm{x_{k+1}-\wh{x}_k}{}{2} - H_f\gnorm{x_{k+1}-\wh{x}_k}{}{} + f(x)
	\end{align*}
	Multiplying the last two relations by $y_{k+1}$, noting that $y_{k+1} \ge \mathbf{0}$ and then summing the above relations, we have for all $x \in X$
	\begin{align*}
		f(x_{k+1}) -f(x) &+ \inprod{y_{k+1}}{\ell_g(x_{k+1}) - g(x)}-  \tfrac{L_f}{2}\gnorm{x_{k+1}-\wh{x}_k}{}{2} - H_f\gnorm{x_{k+1}-\wh{x}_k}{}{} + \tfrac{\mu_f\|x-\hat{x}_k\|^2}{2} \\
		&\le \inprod{f'(\wh{x}_k) + g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x}. 
	\end{align*}
	Using the above relation inside \eqref{eq:int_rel2}, we have for all $x\in X$
	\begin{equation}\label{eq:int_rel4}
		\begin{split}
			f(x_{k+1}) -& f(x) + \inprod{y_{k+1}}{\ell_g(x_{k+1}) -g(x)}+\inner{\delta_k }{\hat{x}_k-x} +\chi_0(x_{k+1}) - \chi_0(x) + \inner{\chi(x_{k+1})-\chi(x))}{y_{k+1}}\\ &\le  \tfrac{(L_k-\mu_f)\gnorm{x-\wh{x}_k}{}{2}}{2}- \tfrac{L_k\gnorm{x-x_{k+1}}{}{2}}{2}
			- \tfrac{L_k-L_f\gnorm{x_{k+1}-\wh{x}_k}{}{2}}{2} + H_f\gnorm{x_{k+1}-\wh{x}_k}{}{}+\inner{\delta_k}{\hat{x}_k-x_{k+1}}.
		\end{split}
	\end{equation}
	Similarly, using first-order optimality condition of $s_{k+1}$ and noting $y_{k+1}\geq \mathbf{0}$, we have for all $s \le \mathbf{0}$, 
	\begin{equation}\label{eq:int_rel3}
		\inprod{y_{k+1}}{s - s_{k+1}} \le 0.
	\end{equation}
	Also, let us consider these two equations 
	\begin{equation}\label{eq:recurtion}
		\begin{aligned}
			&(1-\tau_k)\|x_{k+1} - x_{k}\|^2 + \tau_k\|x_{k+1}-x\|^2 = \|x_{k+1}-(1-\tau_k)x_k-\tau_kx\|^2 + \tau_k(1-\tau_k)\|x_k-x\|^2,\\
			&(1-\tau_k)\|\hat{x}_k - x_{k}\|^2 + \tau_k\|\hat{x}_k-x\|^2 = \|\hat{x}_k-(1-\tau_k)x_k-\tau_kx\|^2 + \tau_k(1-\tau_k)\|x_k-x\|^2,\quad \forall x\in X.
		\end{aligned}
	\end{equation}
	Now, we sum the following four relations: (1) Multiply \eqref{eq:int_rel4} by $\tau_k \in (0,1]$, (2) multiply \eqref{eq:int_rel3} by $\tau_k$, (3) use $x=x_k$ in \eqref{eq:int_rel4} and multiply by $1-\tau_k$, and (4) use $s= s_k$ in \eqref{eq:int_rel3} and multiply by $1-\tau_k$. Then regarding \eqref{eq:recurtion}, we have for all $x \in X, s \le \mathbf{0}$
	\begin{align}
		&f(x_{k+1}) + \chi_0(x_{k+1}) - \tau_k(f(x)+ \chi_0(x)) -(1-\tau_k)(f(x_k)+ \chi_0(x_k))+\inner{\delta_k }{\hat{x}_k-\tau_kx - (1-\tau_k)x_k}\label{eq:int_rel5}\\
		&\quad  + \inprod{y_{k+1}}{\ell_g(x_{k+1})+ \chi(x_{k+1}) - s_{k+1} - \tau_k (g(x)+\chi(x)-s) - (1-\tau_k)(g(x_k)+\chi(x_k)-s_k)}\nonumber\\
		& \le  \tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}\nonumber\\
		&\quad - \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2 - \tfrac{L_k-L_f}{2}\gnorm{x_{k+1} - \wh{x}_k}{}{2} +  H_f\gnorm{x_{k+1}-\wh{x}_k}{}{}+\inner{\delta_k}{\hat{x}_k-x_{k+1}}\nonumber.
	\end{align}
	Finally, noting that $\wt{y}_{k+1} = \argmin_{y} -\inprod{\wt{V}_{k+1} - (1-\tau_k)V_k}{y} + \tfrac{1}{2\eta_k} \gnorm{y-\wt{y}_k}{}{2}$, we have
	\begin{align*}
		\inprod{\wt{V}_{k+1} - (1-\tau_k)V_k}{y-\wt{y}_{k+1}} \le \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} - \gnorm{\wt{y}_{k+1}-\wt{y}_k}{}{2}].
	\end{align*}
	Adding the above relation with \eqref{eq:int_rel5} and noting definitions of $\wt{V}_{k+1}, V_k$ with respect to \eqref{eq:Denotes},  we have
	\begin{equation}\label{eq:int_rel6}
		\begin{aligned}
			&f(x_{k+1}) + \chi_0(x_{k+1}) - \tau_k(f(x)+ \chi_0(x)) -(1-\tau_k)(f(x_k)+ \chi_0(x_k))+\inner{\delta_k }{\hat{x}_k-\tau_kx - (1-\tau_k)x_k}\\
			&\quad-\inprod{\tau_k y_{k+1}}{g(x)+\chi(x)-s} + \inprod{y}{\wt{V}_{k+1} - (1-\tau_k)V_k}\\
			& \le \inprod{\wt{y}_{k+1}-y_{k+1}}{\wt{V}_{k+1} - (1-\tau_k)V_k} - \tfrac{L_k-L_f}{2}\gnorm{x_{k+1} - \wh{x}_k}{}{2} +  H_f\gnorm{x_{k+1}-\wh{x}_k}{}{}\\
			&\quad +\tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}\\
			&\quad + \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} - \gnorm{\wt{y}_{k+1}-\wt{y}_k}{}{2}]+\inner{\delta_k }{\hat{x}_k-x_{k+1}}- \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2.
		\end{aligned}
	\end{equation}
	From the definitions of $y_{k+1}$ and $\wt{y}_{k+1}$ in \eqref{eq:conceptual-x-s-update}and \eqref{eq:Denotes} of Algorithm \ref{alg:augConEx}, we have 
	$\inprod{\wt{y}_{k+1}-y_{k+1}}{\wt{V}_{k+1} - (1-\tau_k)V_k} = (\eta_k-\rho_k) \gnorm{\wt{V}_{k+1} - (1-\tau_k)V_k}{}{2}$. Moreover, $-\tfrac{1}{2\eta_k}\gnorm{\wt{y}_{k+1} - \wt{y}_k}{}{2} = -\tfrac{\eta_k}{2}\gnorm{\wt{V}_{k+1} - (1-\tau_k)V_k}{}{2}$. Using these two relations in \eqref{eq:int_rel6}, alongside with \eqref{eq:conjugate} and Cauchy-Schwarz inequality for $\inner{\delta_k }{\hat{x}_k-x_{k+1}}$ we have 
	\begin{align*}
		&\Lcal(x_{k+1}, s_{k+1}, y) - \Lcal(x,s,\wb{y}_{k+1}) - (1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)] \\
		& \le \tfrac{\eta_k - 2\rho_k}{2}\gnorm{\wt{V}_{k+1} - (1-\tau_k)V_k}{}{2} - \tfrac{L_k-L_f}{2}\gnorm{x_{k+1} - \wh{x}_k}{}{2} +  (H_f+\|\delta_k\|)\gnorm{x_{k+1}-\wh{x}_k}{}{}\nonumber\\
		&\quad +\tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}- \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2 \nonumber\\
		&\quad + \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} ] + \inprod{y}{g(x_{k+1}) - \ell_g(x_{k+1})}-\inner{\delta_k }{\hat{x}_k-\tau_kx - (1-\tau_k)x_k}.
	\end{align*}
	Considering the following relations, one can conclude the proof
	\begin{subequations}
		\begin{equation*}
			(H_f+\|\delta_k\|)\gnorm{x_{k+1}-\wh{x}_k}{}{}\nonumber \leq \tfrac{L_k\gnorm{x_{k+1}-\wh{x}_k}{}{2}\nonumber}{4} + \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k},
		\end{equation*}
		\begin{equation*}
			\begin{aligned}
				\langle y , g(x_{k+1})- \ell_g(x_{k+1})\rangle \leq& \tfrac{L_g}{2}  \| y\| \| x_{k+1}- \hat{x}_k\|^2 + H_g\|y\|\| x_{k+1}- \hat{x}_k\|, \\
				& = \tfrac{L_g}{2} (\| y\| - B)\| x_{k+1}- \hat{x}_k\|^2 + \tfrac{B L_g}{2}\| x_{k+1} - \hat{x}_k\|^2 + H_g\|y\|\| x_{k+1}- \hat{x}_k\|,\\
				& \leq (L_gD_x [\| y\| - B]_++H_g\|y\|) \| x_{k+1}- \hat{x}_k\| + \tfrac{B L_g}{2}\| x_{k+1} - \hat{x}_k\|^2,
			\end{aligned}
		\end{equation*}
		\begin{equation*}
			(L_gD_x  [\| y\| - B]_++H_g\|y\|) \| x_{k+1}- x_k\| - \tfrac{L_k-2(L_f + BL_g)}{4} \| x_{k+1}- \hat{x}_k\|^2\leq \tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}.
		\end{equation*}
	\end{subequations}
\end{proof}
Lemma \ref{lemma:importantlemma} is crucial to obtain optimality and feasibility gaps in Definition \ref{def:gaps}. Indeed, we use Lemma \ref{lemma:importantlemma} to construct convergence results for convex and strongly-convex setting of optimization problem in \ref{eq:prima-problem}. In the following section, we provide the detailed technical results we used to obtain Theorem \ref{thm:convex-case}. 
\subsection{Convergence analysis for the convex problem}
\paragraph{Proof of Theorem \ref{thm:convex-case}}
	First, assume the following conditions for the convex problem
	\begin{equation}\label{eq:conditions}
		\tfrac{\eta_k}{2}\leq \rho_k, \quad L_k\geq 2(L_f+ BL_g + \rho_k(M_g+M_\chi)^2),\quad \tfrac{1}{\eta_k}\leq \tfrac{1-\tau_k}{\eta_{k-1}}.
	\end{equation}
	Thus, one can easily varefiy that the step-size policy in \eqref{eq:non-ergo-stepsize-non-smooth-eta} satisfies the conditions in \eqref{eq:conditions} for $k\geq 2$. 
	Second, letting $\tilde{x}_k  = \tfrac{1}{\tau_k}[\hat{x}_k-(1-\tau_k)x_k]$ and $\tilde{x}_{k+1}  = \tfrac{1}{\tau_k}[x_{k+1}-(1-\tau_k)x_k]$, and taking the expectation from both sides regarding \eqref{eq:SO_F_objective}, we can write the following recursion for $k\geq 2$
	\begin{equation}\label{eq:non-ergo-5-non-smooth-recur-eta}
		\begin{aligned}
			&\Ebb[\Lcal(x_{k+1},s_{k+1}, y)- \Lcal(x,s,\bar{y}_{k+1})  + \tfrac{1}{2\eta_k}\|\tilde{y}_{k+1}-y\|^2]\leq \Ebb\big[
			(1-\tau_k)[ \Lcal(x_{k},s_{k}, y)- \Lcal(x,s,\bar{y}_{k})
			+  \tfrac{1}{2\eta_{k-1}}\|\tilde{y}_k-y\|^2\big]\\
			&+\Ebb\big[\tfrac{\tau_k^2L_k}{2}[\|\tilde{x}_k-x\|^2- \|\tilde{x}_{k+1}-x\|^2]\big] -\tau_k\Ebb[\inner{\delta_k }{\dot{x}_k-x}]
			+ \Ebb\big[ \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}\big]+ \tfrac{2(H_f^2+ \sigma^2)}{L_k}.
		\end{aligned}
	\end{equation}
	Consequently, one can write the following recursion 
	\begin{equation}\label{eq:recur-nonsmooth-eta}
		\begin{aligned}
			&\Ebb[\Lcal(x_{K},s_{K}, y)- \Lcal(x,s,\bar{y}_{K})] \leq  [\prod_{k=2}^{K-1}(1-\tau_k)]\Ebb[\Lcal(x_{2},s_{2}, y)- \Lcal(x,s,\bar{y}_{2})+ \tfrac{1}{2\eta_{1}}\|\tilde{y}_2-y\|^2]\\
			& \quad  +\Ebb\big[ \sum_{k=2}^{K-1} [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tfrac{\tau_k^2L_k}{2}[\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big] -\Ebb\big[\sum_{k=2}^{K-1}[\prod_{i=k+1}^{K-1}(1-\tau_{i})]\tau_k\inner{\delta_k}{\dot{x}_k-x}\big] \\
			& \quad + \sum_{k=2}^{K-1}\big[[ \prod_{i=k+1}^{K-1} (1-\tau_{i})] \Ebb\big[ \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}\big] + \tfrac{2(H_f^2+ \sigma^2)}{L_k}\big].
		\end{aligned}
	\end{equation}
	Now, let us simplify each line in the RHS of \eqref{eq:recur-nonsmooth-eta}. Note that from Lemma \ref{lemma:importantlemma} and $L_1 = L, \eta_{1} = \tfrac{\rho_{1}}{K}, \hat{x}_1 = x_1 , \tilde{y}_1 = y_1, \tau_1=1$ , we have 
	\begin{equation*}
		\begin{aligned}
			\Ebb&[\Lcal(x_{2},s_{2}, y)-\Lcal(x,s,\bar{y}_{2})+ \tfrac{1}{2\eta_{1}}\|\tilde{y}_2-y\|^2]\leq (1-\tau_1)\Ebb[(\Lcal(x_{1},s_{1}, y)- \Lcal(x,s,\bar{y}_{1}))]\\
			& \quad + 2D_X^2 + \tfrac{K}{2\rho_{1}}\Ebb[\|y_1 - y\|^2] + \Ebb\big[\tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{8\rho_1K(M_g + M_\chi)^2}\big] + \tfrac{H_f^2 + \sigma^2}{\rho_1K(M_g + M_\chi)^2} - \Ebb[\inner{\delta_1}{\dot{x}_1-x}].
		\end{aligned}
	\end{equation*}
	Noting that $\tau_1 = 1$ and $\prod_{k=2}^{K-1}(1-\tau_k) = \tfrac{2}{K(K-1)}$ we have the following relation for the first line in RHS of \eqref{eq:recur-nonsmooth-eta}
	\begin{equation}\label{eq:first summation}
		\begin{aligned}
			[\prod_{k=2}^{K-1}(1-\tau_k)]&\Ebb[\Lcal(x_{2},s_{2}, y)- \Lcal(x,s,\bar{y}_{2})+ \tfrac{1}{2\eta_{1}}\|\tilde{y}_2-y\|^2]\leq \tfrac{4LD_X^2}{K(K-1)} + \tfrac{1}{(K-1)\rho_1}\Ebb[\|y_1 - y\|^2]\\
			&\quad +\Ebb\big[\tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4K^2(K-1)\rho_1(M_g + M_\chi)^2}\big]+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2} - \tfrac{2\Ebb[\inner{\delta_1}{\dot{x}_1-x}]}{K(K-1)},
		\end{aligned}
	\end{equation}
	For the first summation  in the second line of \eqref{eq:recur-nonsmooth-eta} we have 
	\begin{equation}\label{eq:second summation}
		\begin{aligned}
			\Ebb\big(\sum_{k=2}^{K-2}& [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tfrac{\tau_k^2L_k}{2}[\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big) +\Ebb\bracket[\big]{\tfrac{\tau_{K-1}^2L_{K-1}}{2}[\|\tilde{x}_{K-1}-x\|^2-\|\tilde{x}_{K}-x\|^2]}\\
			&  \leq \Ebb\big( \sum_{k=2}^{K-2} \tfrac{ k (k+1)}{(K-1)K} \tfrac{4}{(k+1)^2} \tfrac{ L}{2}[\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big) + \tfrac{4D_X^2L}{K^2} \\
			& = \Ebb\big(\sum_{k=2}^{K-2} \tfrac{2 k }{(K-1)K (k+1)} L [\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big) + \tfrac{4D_X^2L}{K^2}\\
			& = \tfrac{2L}{(K-1)K}\Ebb \Big(\big(\sum_{k=2}^{K-2} \big[\tfrac{k+1}{k+2}
			-\tfrac{k}{k+1}\big] \|\tilde{x}_{k+1}-x\|^2 \big)+ \tfrac{1}{2}  \|\tilde{x}_{1}-x\|^2\Big) + \tfrac{4D_X^2L}{K^2} \\
			&  = \tfrac{2L}{(K-1)K} \sum_{k=2}^{K-2} \big(\tfrac{k+1}{k+2} - \tfrac{k}{k+1}\big) \Ebb(\|\tilde{x}_{k+1}-x\|^2)  + \tfrac{L}{(K-1)K}  \|\tilde{x}_{1}-x\|^2 + \tfrac{4D_X^2L}{K^2}\\
			& \leq  \tfrac{8L}{(K-1)K} D_x^2 + \tfrac{4L}{(K-1)K} D_x^2 + \tfrac{4L}{K^2}D_X^2\leq  \tfrac{16L}{(K-1)K}D_X^2
		\end{aligned}
	\end{equation}
	The last summation line in the RHS of \eqref{eq:recur-nonsmooth-eta} has the following upper bound.
	\begin{equation}\label{eq:third summation}
		\begin{aligned}
			&\sum_{k=2}^{K-2}\big[[ \prod_{i=k+1}^{K-1} (1-\tau_{i})] \Ebb\big[ \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}\big] + \tfrac{2(H_f^2+ \sigma^2)}{L_k}\big] + \big[\Ebb[\tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4(L_{K-1}-2(L_f+ BL_g ))}] + \tfrac{2(H_f^2+ \sigma^2)}{L_{K-1}}\big]\\
			& = \Big(\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(K-1)K(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{(K-1)KL}\Big) \sum_{k=2}^{K-2} k(k+1)  + \big[\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{L}\big]\\
			&  \leq \Big(\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(K-1)K(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{(K-1)KL}\Big) \tfrac{ (K-1)^3}{3} + \big[\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{L}\big] \\
			& \leq  \tfrac{K\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{12(L-2(L_f+ BL_g ))} +\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} +  \tfrac{2K(H_f^2+ \sigma^2)}{3L}+ \tfrac{2(H_f^2+ \sigma^2)}{L}
		\end{aligned}
	\end{equation} 
	
	Thus from \eqref{eq:first summation}, \eqref{eq:second summation}, and \eqref{eq:third summation}, the recursion in \eqref{eq:recur-nonsmooth-eta} can be written as follows 
	\begin{equation}\label{eq:recur-nonsmooth-eta-4}
		\begin{aligned}
			&\Ebb(\Lcal(x_{K},s_{K}, y)- \Lcal(x,s,\bar{y}_{K})) \leq  \tfrac{20L}{(K-1)K}D_X^2 + \tfrac{1}{(K-1)\rho_{1}}\Ebb[\|y_1 - y\|^2]  + \tfrac{K(8(H_f^2+ \sigma^2) +\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2] )}{12(L-2(L_f+ BL_g ))} \\
			& \quad+ \tfrac{8(H_f^2+ \sigma^2) +\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} +\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4K^2(K-1)\rho_1(M_g + M_\chi)^2}+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}\\
			&-\Ebb\big[\sum_{k=2}^{K-1}[\prod_{i=k+1}^{K-1}(1-\tau_{i})]\tau_k\inner{\delta_k}{\dot{x}_k-x}\big]  - \tfrac{2\Ebb[\inner{\delta_1}{\dot{x}_1-x}]}{K(K-1)}  .
		\end{aligned}
	\end{equation}
	We know that $ \Lcal(x_K,y)\leq \Lcal(x_K,s_K,y)$ and for $s =0$ we have $\Lcal(x,\bar{y}_K) = \Lcal(x,0,\bar{y}_K)$. Therefore, we have the following
	\begin{equation}\label{eq:conjugate-1}
		\Lcal(x_K,y) - \Lcal(x,\bar{y}_K) \leq \Lcal(x_K,s_K,y) - \Lcal(x,0,\bar{y}_K) \quad \forall (x,y)\in X\times \mathbb{R}^m_+.
	\end{equation}
	Now, let us choose $ y =0 $. we know $ \bar{y}_K\geq 0$ and $\psi(x^*)\leq 0$ thus $ \langle \bar{y}_K, \psi(x^*)\rangle \leq 0 $. Also note that $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0$. Therefore, regarding \eqref{eq:recur-nonsmooth-eta-4} and \eqref{eq:conjugate-1}, we have
	\begin{equation*}\label{eq:optimality-gap}
		\Ebb[\psi_0(x_K)- \psi_0(x^*)]\leq\tfrac{		20L}{(K-1)K}D_X^2+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 \|^2 + \tfrac{8(K+3)(H_f^2+ \sigma^2)}{12(L-2(L_f+ BL_g ))}+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2},
	\end{equation*}
	Applying the step-size policy in \eqref{eq:non-ergo-stepsize-non-smooth-eta} we obtain 
	\begin{equation*}
		\begin{aligned}
			\Ebb[\psi_0(x_K)- \psi_0(x^*)]\leq&\tfrac{D_X\sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+ \sigma^2))}}{6(K-1)}+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 \|^2 + \tfrac{40D_X^2(L_f+ BL_g +\rho_{1} K(M_g + M_\chi)^2)}{(K-1)K}\\
			& \quad+\tfrac{80D_X(K+3)(H_f^2+ \sigma^2)}{K(240D_X\rho_{1}(M_g+M_\chi)^2 + \sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+\sigma^2))})}+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}.
		\end{aligned}
	\end{equation*}
	Now, let us move to the feasibility gap. First, observe that 
	\begin{equation*}\label{eq:first-frasib}
		\Lcal(x_K,y^*) - \Lcal(x^*,y^*)\geq 0
	\end{equation*}
	
	implying that 
	\begin{equation*}\label{eq:second-feasib}
		\psi_0(x_K) + \inner{y^*}{\chi(x_K)} - \psi_0(x^*)\geq 0 ,
	\end{equation*}
	
	which in the view of below relation 
	\begin{equation*}\label{eq:feasib3}
		\inner{y^*}{\psi(x_K)}\leq \inner{y^*}{[\psi(x_K)]_+}\leq \|y^*\|\|[\psi(x_K)]_+\|
	\end{equation*}
	
	we have 
	\begin{equation}\label{eq:haty}
		\psi_0(x_K) +\|y^*\|\|[\psi(x_K)]_+\| - \psi_0(x^*)\geq 0.
	\end{equation}
	Moreover, $\Lcal(x_K,\hat{y})-\Lcal(x^*,\bar{y}_K)\geq\Lcal(x_K,\hat{y})-\Lcal(x^*,y^*) = \psi_0(x_K) +(\|y^*\|+1)\|[\psi(x_K)]_+\| - \psi_0(x^*)$. Therefore,  considering \eqref{eq:conjugate-1}, \eqref{eq:haty}, $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0 $, and the definition of $\hat{y}$ as $\hat{y} = (\|y^*\|+1)\tfrac{[g(\bar{x}_K)]_+}{\|[g(\bar{x}_K)]_+\|}$, the feasibility gap can be written as 
	\begin{equation*}
		\begin{aligned}
			\Ebb(\|[\psi(x_K)]_+\|)\leq  \Ebb(\Lcal(x_K,\hat{y})- &\Lcal(x^*,\bar{y}_K)) \leq  \tfrac{D_X\sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+ \sigma^2))}}{6(K-1)} + \tfrac{40D_X^2(L_f+ BL_g + \rho_{1}K(M_g + M_\chi)^2)}{(K-1)K}\\
			& \quad + \tfrac{80D_X(K+3)(8(H_f^2+ \sigma^2) +\mathcal{H}_*^2 )}{K(240D_X\rho_{1}(M_g+M_\chi)^2 + \sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+\sigma^2))})}+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 - \hat{y} \|^2 \\
			&\quad +\tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}
		\end{aligned}
	\end{equation*}  
\subsection{Convergence analysis for the strongly convex case}
Before stating the convergence results for the strongly convex case, let us mention the following lemma  
\begin{lemma}\label{lemma:Dinh's strong}
	(Lemma 15 of \cite{blah}) Given \( \mu_f \geq 0 \), \( L_k \geq \mu_f \), and \( \tau_{k} \in (0,1) \), let \( m_k := \tfrac{L_k}{L_{k-1}} \) and \( \{x_k\}\) be a given sequence in \( \mathbb{R}^n \). We define \( \hat{x}_k := x_k + \beta_k \left( x_k - x_{k-1} \right) \), where \( \beta_k := \tfrac{(1 - \tau_{k-1})\tau_{k-1}}{\tau_{k-1}^2+m_k\tau_{k}} \).
	
	Assume that the following two conditions hold:
	\begin{subequations}\label{eq:lemma15-cond}
		\begin{equation}
			L_{k-1} (1-\tau_{k})\tau_{k-1}^2 + \mu_f(1-\tau_{k})\tau_{k} \geq (L_k-\mu_f)\tau_{k}^2,
		\end{equation}
		\begin{equation}
		L_{k-1} (\tau_{k-1}^2+ m_k\tau_{k})m_k\tau_{k}\geq (L_k-\mu_f)\tau_{k-1}^2.
	\end{equation}
	\end{subequations}
	Then, for any \( x \in \mathbb{R}^k \), we have
	\[
	(L_k-\mu_f)\tau_{k}^2\gnorm{\tfrac{1}{\tau_{k}}[\hat{x}_k-(1-\tau_{k})x_k]-x}{}{2} - \mu_f\tau_{k}(1-\tau_{k})\gnorm{x_k-x}{}{2}\leq 	L_{k-1} (1-\tau_{k})\tau_{k-1}^2\gnorm{\tfrac{1}{\tau_{k-1}}[x_k-(1-\tau_{k-1})x_{k-1}]-x}{}{2}. 
	\]
	
\end{lemma}
Now, we are ready to mention the proof of Theorem \ref{thm:non-ergo-strong-semi}. 	
\paragraph{Proof of Theorem \ref{thm:non-ergo-strong-semi}.}
	First of all, the updates in \eqref{eq:non-ergo-stepsize-strong} leads to the following equations for all $k\geq 2$
	\begin{equation*}\label{eq:relations-last-iter}
		\tau_k^2 = (1-\tau_k)\tau_{k-1}^2, \quad \tfrac{1}{k+1}\leq \tau_{k}\leq\tfrac{2}{k+1}.
	\end{equation*}
	Thus, $\rho_{k-1} = \tfrac{\rho_{1}}{\tau_{k-1}^2} = \tfrac{(1-\tau_k)\rho_1}{\tau_k^2} = (1-\tau_k)\rho_k$ which implies 
	\begin{equation*}\label{eq:relations-last-iter-2}
	 \tfrac{1}{\eta_k}= \tfrac{1-\tau_k}{\eta_{k-1}}, \quad \forall k\geq 2.
	\end{equation*}
	Also, note $\eta_k<2\rho_k $ and $L_{k}$ satisfies the conditions in Lemma \ref{lem:F-contraction} and Lemma \ref{lemma:importantlemma} implying all the conditions in these lemmas hold. In addition, since $0< \rho_1=\tfrac{\mu_f}{(M_g + M_\chi)^2}$, and $\{\beta_{k}\}_{k\geq2}$ in \eqref{eq:non-ergo-stepsize-strong} is defined as Lemma \ref{lemma:Dinh's strong}, then all conditions in Lemma \ref{lemma:Dinh's strong} including \eqref{eq:lemma15-cond} hold for all $k\geq 2$.
	Hence using Lemma \ref{lemma:Dinh's strong}, we have the following useful relation for any $x\in X$. 
	\begin{equation}\label{eq:resultlemma15}
		\begin{aligned}
			&(L_k-\mu_f)\tau_k^2\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2}-\mu_f(1-\tau_k)\tau_k\|x_k-x\|^2\\
			\leq &(1-\tau_k)L_{k-1}\tau_{k-1}^2\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}, \quad \forall k\geq 2,
		\end{aligned}
	\end{equation}
	Now, substituting \eqref{eq:resultlemma15} into Lemma \ref{lemma:importantlemma}, one can obtain the following result for all $k\geq 2$
	\begin{equation}\label{eq:recur1}
		\begin{aligned}
			\Lcal(x_{k+1}, s_{k+1}, y) -& \Lcal(x,s,\wb{y}_{k+1})  
			\le(1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)]\\
			&+\tfrac{(1-\tau_k)L_{k-1}\tau_{k-1}^2}{2}\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}\\
			&\quad - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}   + \tfrac{1-\tau_k}{2\eta_{k-1}}\gnorm{y-\wt{y}_k}{}{2} -\tfrac{1}{2\eta_k} \gnorm{y-\wt{y}_{k+1}}{}{2}\\
			&\quad  + \tfrac{(L_gD_x[\|y\|-B]_+ + H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}-\tau_k\inner{\delta_k }{\dot{x}_k-x}.
		\end{aligned}
	\end{equation}
	By rearranging \eqref{eq:recur1} we have the following result 
	\begin{equation}\label{eq:recur2}
		\begin{aligned}
			\Lcal(x_{k+1}, &s_{k+1}, y) - \Lcal(x,s,\wb{y}_{k+1})+\tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}+ \tfrac{1}{2\eta_k} \gnorm{y-\wt{y}_{k+1}}{}{2}  \\
			&\le(1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)+\tfrac{L_{k-1}\tau_{k-1}^2}{2}\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}\\
			&\quad + \tfrac{1}{2\eta_{k-1}}\gnorm{y-\wt{y}_k}{}{2} ] -\tau_{k}\inner{\delta_k }{\dot{x}_k-x} + \tfrac{(L_gD_x[\|y\|-B]_+ + H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k} .
		\end{aligned}
	\end{equation}
	Let us consider $Q_k(x,y)$ s follows 
	\[
	Q_k(x,y)  = \Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)+\tfrac{L_{k-1}\tau_{k-1}^2}{2}\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}+ \tfrac{1}{2\eta_{k-1}}\gnorm{y-\wt{y}_k}{}{2}.
	\]
	Hence \eqref{eq:recur2} implies the following 
	\begin{equation}\label{eq:Q_recur}
		Q_{k+1}(x,y)\leq (1-\tau_k)Q_k(x,y)  +  \tau_{k}\inner{\delta_k }{x-\dot{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}, \quad \forall k\geq 2.
	\end{equation}
	Moreover regarding  initialization in Algorithm \ref{alg:augConEx}, Lemma \ref{lemma:importantlemma} and the step-size policy in Theorem \ref{thm:non-ergo-strong-semi}, we have the following relations for $k=2$ 
	\begin{equation}\label{eq:Q_1}
		Q_2(x,y)\leq \tfrac{L_1-\mu_f}{2}\|x_1-x\|^2 + \tfrac{1}{2\eta_{1}}\|y_1-y\|^2+ \tfrac{(L_gD_x[\|y\|-B]_+ + H_g\|y\|)^2}{4(L_1-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_1\|^2)}{L_1}-\inner{\delta_1 }{\dot{x}_1-x}.
	\end{equation}
	Using the recursion in \eqref{eq:Q_recur} from $k=2$ to $K-1$ and considering $\tau_1 =1, \tilde{y}_1 = y_1$, and $ \hat{x}_1 = x_1$ we have 
	\begin{equation}\label{eq:recur3}
		\begin{aligned}
			\Lcal(x_{K}, &s_{K}, y) - \Lcal(x,s,\wb{y}_{K}) 
			\le[\prod_{k=2}^{K-1} (1-\tau_{k})]Q_2(x,y)
			\\
			&\quad +\sum_{k=2}^{K-1}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})]\tau_{k} \inner{\delta_k }{x-\dot{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big]\\
			&\leq \tfrac{4}{(K+1)^2}[(L_f+BL_g)\|x_1-x\|^2+ \tfrac{1}{2\eta_{1}}\|y_1-y\|^2 + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4\rho_{1}(M_g+M_\chi)^2}\\
			&\quad+\tfrac{H_f^2+\|\delta_1\|^2}{(L_f+BL_g+\rho_{1}(M_g + M_\chi^2))} - \inner{\delta_1}{\dot{x}_1-x}] +\inner{\delta_{K-1}}{x-\hat{x}_{K-1}} + \tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4(L_{K-1}-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \|\delta_{K-1}\|^2)}{L_{K-1}}\\
			&\quad	 +\sum_{k=2}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tau_{k}\inner{\delta_k }{x-\hat{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big],
		\end{aligned}
	\end{equation}
	where we used \eqref{eq:Q_1}, $\rho_{1}(M_g+M_{\chi})^2= \mu_f$  and $[\prod_{k=2}^{K-1} (1-\tau_{k})] = \tfrac{\tau_{K-1}^2}{\tau_1}\leq \tfrac{4}{(K+1)^2}$ to obtain the second inequality. 	
	We know that $ \Lcal(x_K,y)\leq \Lcal(x_K,s_K,y)$ and for $s =0 $, we have $\Lcal(x,\bar{y}_K) = \Lcal(x,0,\bar{y}_K)$ leading to the following relation 
	\begin{equation}\label{eq:relation3}
		\Lcal(x_K,y) - \Lcal(x,\bar{y}_K) \leq \Lcal(x_K,s_K,y) - \Lcal(x,0,\bar{y}_K).
	\end{equation}
	Using \eqref{eq:relation3}, with \eqref{eq:recur3} alongside definition of $  \Lcal(x,y)$ we have 
	\begin{equation}\label{eq:non-ergo-8}
		\begin{aligned}
			&\psi_0(x_K)+ \langle y , \psi(x_K)\rangle - \psi_0(x) - \langle \bar{y}_K, \psi(x)\rangle \leq  \tfrac{4}{(K+1)^2}[(L_f+BL_g)\|x_1-x\|^2\\
			&\quad+ \tfrac{1}{2\eta_{1}}\|y_1-y\|^2+\tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2 +4(H_f^2+\|\delta_1\|^2)}{4\rho_{1}(M_g+M_\chi)^2)}- \inner{\delta_1}{\dot{x}_1-x}]
			\\&\quad +\sum_{k=2}^{K-1}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tau_{k}\inner{\delta_k }{x-\dot{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big]
		\end{aligned}
	\end{equation}
	Now let us choose $ y =0 $. we know $ \bar{y}_K\geq 0$ and $\psi(x^*)\leq 0$, thus $ \langle \bar{y}_K, \psi(x^\ast)\rangle \leq 0 $. Rewriting \eqref{eq:non-ergo-8} for $(x,y)=(x^*,0)$ and taking the expectation from both sides with respect to $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0 $, one can conclude the following 
	\begin{equation}\label{eq:feasib}
		\begin{aligned}
			\Ebb[\psi_0(x_K) - \psi(x^*)]\leq& \tfrac{4}{(K+1)^2}[(L_f+BL_g)4D_X^2
			+ \tfrac{1}{2\eta_{1}}\|y_1\|^2 + \tfrac{(H_f^2+\sigma^2)}{\rho_{1}(M_g+M_\chi)^2} ]\\
			&\quad	+\sum_{k=2}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})]  \tfrac{2(H_f^2+\sigma^2)}{L_k}\big] + \tfrac{H_f^2+ \sigma^2}{\rho_{K-1}(M_g+M_\chi)^2}.
		\end{aligned}
	\end{equation}
	Now let us focus on the following summation 
	\begin{equation}\label{eq:first-sum}
		\begin{aligned}
			\sum_{k=2}^{K-2} [\prod_{i=k+1}^{K-1} (1-\tau_{i})]\tfrac{2(H_f^2+\sigma^2)}{L_k}
			&\leq \sum_{k=2}^{K-2} \tfrac{\tau_{K-1}^2}{\tau_{k}^2}\tfrac{H_f^2+\sigma^2}{\rho_k (M_g+M_\chi)^2} \leq \tfrac{4(H_f^2+\sigma^2)}{(K+1)^2}\sum_{k=2}^{K-2} \tfrac{1}{\rho_1 (M_g+M_\chi)^2} \leq\tfrac{4K(H_f^2+\sigma^2)}{(K+1)^2\mu_f},
		\end{aligned}
	\end{equation}
	where we used $\tfrac{1}{k+1}\leq \tau_k\leq\tfrac{2}{k+1}$ and $\rho_{1}(M_g+M_\chi)^2=\mu_f$ in the last two inequalities. Moreover, note that $\tfrac{H_f^2+ \sigma^2}{\rho_{K-1}(M_g+M_\chi)^2} = \tfrac{4(H_f^2+\sigma^2)}{(K+1)^2\mu_f}$.Therefore, using \eqref{eq:feasib} and \eqref{eq:first-sum}, we concludes \eqref{eq:opt-1-non-ergo}.
	Now let us focus on the feasibility convergence rate. First, we rewrite \eqref{eq:non-ergo-8} for any $ x=x^*$ and $\hat{y}$, where $\hat{y} = (\|y^*\|+1)\tfrac{[g(\bar{x}_K)]_+}{\|[g(\bar{x}_K)]_+\|}$.  We have 
	\begin{equation}\label{eq:non-ergo-10}
		\begin{aligned}
			\psi&_0(x_K)+ \langle \hat{y} , \psi(x_K)\rangle - \psi_0(x^*) - \langle \bar{y}_K, \psi(x^*)\rangle \leq  \tfrac{4}{(K+1)^2}[(L_f+BL_g) \|x_1-x^*\|^2\\
			&+ \tfrac{1}{2\eta_{1}}\|y_1-\hat{y}\|^2+\tfrac{\mathcal{H}_*^2 +4(H_f^2+\|\delta_1\|^2)}{4\rho_{1}(M_g+M_\chi)^2} - \inner{\delta_1}{\dot{x}_1-x^*}]+ \big[\tfrac{\mathcal{H}_*^2}{4(L_{K-1}-2(L_f+ BL_g ))}+\inner{\delta_{K-1}}{x^*-\dot{x}_{K-1}}  + \tfrac{2(H_f^2+ \|\delta_k\|^2)}{L_{K-1}}\big]\\
			&\quad
			+\sum_{k=1}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \inner{\delta_k }{x^*-\hat{x}_k} + \tfrac{\mathcal{H}_*^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big]\\
			&.
		\end{aligned}
	\end{equation}
	Using the similar argument in Theorem \ref{thm:convex-case}, one can conclude the following
	\begin{equation}\label{eq:non-ergo-feas-10}
		\begin{aligned}
			\|[ \psi({x}_K)]_+\|& \leq  \tfrac{4}{(K+1)^2}[(L_f+BL_g)\|x_1-x^*\|+ \tfrac{1}{2\eta_{1}}\|y_1-\hat{y}\|^2 
			+ \tfrac{\mathcal{H}_*^2 + 4(H_f^2+\|\delta_k\|^2)}{4\rho_{1}(M_g+M_\chi)^2}+ \inner{\delta_1}{x-\dot{x}_1}]\\
			&\quad+\inner{\delta_{K-1}}{x-\hat{x}_{K-1}}+\big[\tfrac{\mathcal{H}_*^2}{4(L_{K-1}-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \|\delta_{K-1}\|^2)}{L_{K-1}}\big]\\
			&\quad+\sum_{k=1}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \inner{\delta_k }{x-\hat{x}_k} + \tfrac{\mathcal{H}_*^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big].
		\end{aligned}
	\end{equation} 
	Taking the expectation from both sides of \eqref{eq:non-ergo-feas-10} with respect to $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0 $, using similar relations we had in \eqref{eq:first-sum}, and $\rho_{1}(M_g+M_\chi)^2= \mu_f$ one concludes \eqref{eq:feasib-1-non-ergo}. $ \openbox $
	

==> sec-notation.tex <==
\section{Notation and Preliminaries}\label{sec:preliminaries}
We use the following notation throughout the paper. Let $\gnorm{\cdot}{}{}$ represent the standard Euclidean norm. The nonnegative orthant of $\Rbb^k$ is denoted as $\Rbb^k_+$. For the given convex set $X$, we denote its normal cone at $x\in X$ as $N_X(x):=\{v:\inprod{v}{\wt{x}-x}\le 0, \ \forall\ \wt{x} \in X\}$. For the compact set $X$, we denote its diameter $D_X:=\max_{x_1, x_2 \in X}\gnorm{x_1-x_2}{}{}$. Let $g(x) := [g_1(x), \dots, g_m(x)]^T$ and constraints in \eqref{eq:def_X_tilde} can be expressed as $g(x) \le \zero$. Here, bold $\zero$ denotes the vector with all elements being $0$. %The size of vector $\zero$ depends on and is clear from the context. E.g., the size of the vector $\zero$ in the expression $g(x) \le \zero$ is $m$. 
We denote the (sub)gradient of $g_j$ for both smooth or nonsmooth cases by $\grad g_j,\ j = 1, \dots, m$. For each $g_j$, we represent its subdifferential at point $x\in X$ by $\partial g_j(x)$. We define $\grad g(x) := [\grad g_1(x), \dots, \grad g_m(x)] \in \Rbb^{n \times m}$. For any $x\in \Rbb$, we define $[x]_+$ as $\max\{x,0\}$. For a vector $x \in \Rbb^k$, we use $[x]_+$ to denote element-wise application of $[\cdot]_+$. Moreover, the ``+'' operation on sets denotes their Minkowski sum. 

We provide formal definitions for several concepts introduced earlier.  
% We say that  the operator $F:\wt{X}\rightarrow \Rbb^n$ is $L$ Lipschitz (continuous) for some $L>0$ if 
% \[\gnorm{F(x)-F(y)}{2}{}\le \gnorm{x-y}{}{} \quad  \forall x,y\in\wt{X}.\] 
% The associated problem~\eqref{eq:FCVI} is referred to as  a smooth VI. 
% If $F(x)$ is a bounded operator, then problem~\eqref{eq:FCVI} is called a nonsmooth VI. 
%\paragraph{Composite FCVIs}
We consider the general case where $F$ is possibly composed of Lipschitz continuous, and bounded discontinuous monotone operators, satisfying
\begin{equation}\label{eq:F-Lipschitz-property}
	\inprod{F(x_1) - F(x_2)}{x_1-x_2} \le L\gnorm{x_1-x_2}{}{} + H,
\end{equation}
where the $L$-term arises from the Lipschitz continuous component and the $H$-term from the discontinuous component. When $H = 0$, the above definition reduces to Lipschitz continuous operator which is also called as ``smooth operator'' in some VI literature.
We assume that $g_j$ is composed of smooth and nonsmooth components satisfying the following Lipschitz-type property:
\begin{equation}
    \label{eq:g_i-Lipschitz-property}
    g_j(x_1) -g_j(x_2) - \inprod{\grad g_j(x_2)}{x_2-x_1} \le \tfrac{L_{g_j}}{2} \gnorm{x_1-x_2}{}{2} + H_{g_j}\gnorm{x_1-x_2}{}{}, \quad j =1, \dots, m,
\end{equation}
where $L_{g_j}$-term arises from the Lipschitz smooth component of $g_j$ and $H_{g_j}$-term arises from the nonsmooth component of $g_j$. 
Using \eqref{eq:g_i-Lipschitz-property} and Cauchy-Schwarz inequality, it is easy to see that
\begin{equation}
    \label{eq:g-Lipschitz-prop}
    \gnorm{g(x_1) - g(x_2) - \inprod{\grad g(x_2)}{x_1-x_2}}{}{} 
    \le \tfrac{L_g}{2}\gnorm{x_1-x_2}{}{2} + H_g\gnorm{x_1-x_2}{}{},
\end{equation}
where %$\grad g(x^t) =[\grad g_1(x^t) \dots \grad g_m(x^t)] \in \Rbb^{n\times m}$, 
$L_g := \paran{\tsum_{j=1}^m L_{g_j}^2}^{1/2}$ and $H_g := \paran{\tsum_{j=1}^m H_{g_j}^2}^{1/2}$.

In each of the deterministic, stochastic and fully-stochastic settings mentioned earlier, we further classify FCVI problems into smooth and nonsmooth cases as follows:
\begin{enumerate}
    \item Smooth FCVI problem: We say that FCVI problem \eqref{eq:FCVI} is smooth if both operator $F$ and constraint functions $g_j, j =1, \dots, m$ are smooth, i.e., $H = H_{g_1} = \dots = H_{g_m} = 0$. This implies, for the smooth FCVI problem, we have $H = H_g  =0$.
    \item Nonsmooth FCVI problems: The FCVI problems which do not fall into the smooth case (and satisfies relations \eqref{eq:F-Lipschitz-property}, \eqref{eq:g_i-Lipschitz-property}) are called nonsmooth FCVI problems. Hence, at least one of $H > 0$ and $H_g > 0$ must hold for nonsmooth FCVI problems.
\end{enumerate} 
\paragraph{Optimality criteria for FCVIs}
Throughout this paper, we assume that the solution of \eqref{eq:FCVI}, denoted by $x^*$, exists. If the constraint $\{g(x) \le \zero\}$ were not present, then the resulting problem would be a standard VI problem with $\wt{X} = X$. 
Then, by definition of $x^*$, we have the following necessary and sufficient condition for the solution of VI
\[ F(x^*) + N_X(x^*) \ni \zero.\]
In the presence of function constraints $\{g(x) \le 0\}$, this condition can be extended to a KKT form \cite{facchinei2003finite} under an additional constraint qualification such as Slater's condition:  There exists a vector $\lambda^* \in \Rbb^m_+$ such that
\begin{subequations}\label{eq:KKT_opt_FCVI}
	\begin{align}
		F(x^*) + \tsum_{j =1}^m\lambda^*_j \partial g_j(x^*) + N_X(x^*) &\ni \zero;\label{eq:opt_condn_FCVI}\\
		\lambda^*_jg_j(x^*) &= 0, \quad	\forall\ j =1, \dots,m,\label{eq:compl_slackness_condn_FCVI}
	\end{align}
\end{subequations}
where the sum in the first equation is the Minkowski sum of sets. We also assume that $\lambda^*$ exists throughout this paper.
Consider the following Lagrangian function
\begin{equation}\label{eq:Lag_fun_FCVI}
    \Lcal(x, \lambda) := \inprod{F(x^*)}{x} + \inprod{\lambda} {g(x)}.  
\end{equation}
It is easy to see that this is a convex-concave function for $x\in X$ and $\lambda \in \Rbb^m_+$. We denote the gradient or subgradient of $\Lcal$ with respect to the first argument $x$ as $\grad_x \Lcal(x, \lambda)$. Similarly, we express the gradient with respect to the second argument $\lambda$  as $\grad_\lambda\Lcal(x, \lambda)$. We observe that \eqref{eq:KKT_opt_FCVI} is equivalent to
\[ \hspace{4em}\Lcal(x, \lambda^*) \ge \Lcal(x^*, \lambda^*) \ge \Lcal(x^*, \lambda), \quad \forall x \in X, \lambda \in \Rbb^m_+.\]
Indeed, the first inequality is equivalent to \eqref{eq:opt_condn_FCVI} due to the convexity of  $\Lcal(\cdot, \lambda^*)$, and it is easy to see that the second inequality is equivalent to the complementary slackness condition in \eqref{eq:compl_slackness_condn_FCVI}. From the above relation, we see that the pair $(x^*, \lambda^*)$ is 
the saddle point solution of the following min-max problem
\begin{equation}\label{eq:FCVI_SPP_reformulation}
	\min_{x \in X} \max_{\lambda \ge \zero} \Lcal(x, \lambda).
\end{equation}
Based on this discussion, it is clear that the saddle point problem above is an equivalent reformulation of FCVIs~\eqref{eq:FCVI} under the assumption that $(x^*, \lambda^*)$ satisfying \eqref{eq:KKT_opt_FCVI} exists. We state this assumption formally.
\begin{assumption}\label{Assump:Assumption-1}
Throughout this paper, we assume that $(x^*, \lambda^*)$ satisfying \eqref{eq:KKT_opt_FCVI} exists.
\end{assumption}
In the nonlinear programming literature \cite{mangasarian1994nonlinear, bertsekas99nonlinear}, various constraint qualifications are proposed which  are sufficient to ensure the existence of ``dual'' solution $\lambda^*$. Similarly, various constraint qualifications are studied for FCVI problems under the topic of generalized complementarity problems (see the survey article \cite{harker1990finite}).

For the equivalent saddle point reformulation in \eqref{eq:FCVI_SPP_reformulation}, a popular convergence criterion associated with a candidate solution $(\wt{x}, \wt{\lambda}) \in X\times \Rbb^m_+$ is the so called primal-dual gap $\max_{x\in X, \lambda \ge \zero} \Lcal(\wt{x}, \lambda) - \Lcal(x, \wt{\lambda})$. Later, we will show that an $\epsilon$ primal-dual gap corresponds to an $\epsilon$-solution of FCVI problem \eqref{eq:FCVI} (c.f. Definition \ref{def:appx-soln}). Hence, it motivates us to develop primal-dual type algorithms that decrease the primal-dual gap function. Below, we formally define the $\epsilon$-solution of the FCVI problem. We also consider the stochastic case in the following definition.
\begin{definition}\label{def:appx-soln}
	We say that $\wt{x}$ is an $\epsilon$-solution of \eqref{eq:FCVI} if
	\begin{equation}
		\max_{x\in \wt{X}}\,\inprod{F(x)}{\wt{x}-x} \le \epsilon , 
        \quad
		\gnorm{\bracket{g(\wt{x})}_+}{}{} \le \epsilon. 
        \label{eq:weak-VI}
	\end{equation}
    Similarly, we say that $\wt{x}$ is a stochastic $\epsilon$-solution of \eqref{eq:FCVI} if 
    \begin{equation}
		\Ebb\,[\max_{x\in \wt{X}}\,\inprod{F(x)}{\wt{x}-x}] \le \epsilon,
        \quad
		\Ebb\,[\gnorm{\bracket{g(\wt{x})}_+}{}{}] \le \epsilon, 
        \label{eq:stoch_weak-VI}%\\\label{eq:stoch_approx_feasibility}
	\end{equation}
 where the expectation is taken over the randomness of the algorithm used to generate $\wt{x}$.
\end{definition}
When the function constraint $g(x)\le \zero$ is not present, the criteria in \eqref{eq:weak-VI} %, \eqref{eq:approx_feasibility} 
reduces to $\max_{x \in X} \inprod{F(x)}{\wt{x} -x}$. This criterion is commonly referred to as the  ``weak-gap'' in the VI literature for the set-constrained problems~\cite{Nemirovski2004}. Moreover, its stochastic counterpart in \eqref{eq:stoch_weak-VI} %, \eqref{eq:stoch_approx_feasibility} 
reduces to $\Ebb[\max_{x \in X} \inprod{F(x)}{\wt{x} -x}]$, which is a widely adopted stochastic weak-gap criterion in the SVI literature~\cite{Kotsalis2022, boob2021optimal}. 

==> sec-stochastic-opex-method.tex <==
\section{Modified Operator Extrapolation for nonsmooth stochastic FCVIs}


==> sec-stochastic.tex <==
\section{The Aug-ConEx Method  } \label{algorithm}
Before stating the algorithm, we state the fundamental assumptions and problem setup in more details. First, we assume that $f$ and $g_i$, $i\in[m]$  satisfy the following Lipschitz smoothness and non-smoothness respectively. In particular, we have the following
		\begin{equation}\label{eq:smooth-nonsmooth}
		f(x)-f(y) - \inner{f'(y)}{x-y} \le \tfrac{L_f}{2}\gnorm{x-y}{}{2} + H_f\gnorm{x-y}{}{}, \quad \forall x, y\in X,\quad\forall f'(y)\in \partial f(y),
	\end{equation}
where $L_f$ and $H_f$ are the smoothness and non-smoothness constants of $f$. For constraints, we make a similar assumption as in \eqref{eq:smooth-nonsmooth} 
		\begin{equation}\label{eq:sonstraint-smooth-nonsmooth}
	g_i(x)-g_i(y) - \inner{g_i'(y)}{x-y} \le \tfrac{L_{g_i}}{2}\gnorm{x-y}{}{2} + H_{g_i}\gnorm{x-y}{}{}, \quad \forall x, y\in X,\quad\forall g_i'(y)\in \partial g_i(y), i\in [m],
\end{equation}
where $L_{g_i}$ and $H_{g_i}$ are smoothness and non-smoothness constants of the functions $g_i$ for all $i\in[m]$. In addition, we have the following assumptions that the constraint functions are Lipschitz continuous. Specifically, we have the following
 \begin{subequations}\label{eq:M_g}
 	\begin{equation}
 		g_i(x)-g_i(y)\leq M_{g_i}\gnorm{x-y}{}{} \quad \forall x,y\in X\quad i\in [m],
 	\end{equation}
 	\begin{equation}
 		\chi_i(x)-\chi_i(y)\leq M_{\chi_i}\gnorm{x-y}{}{} \quad \forall x,y\in X\quad i \in [m].
 	\end{equation}
 \end{subequations}
Note that the Lipschitz-continuity assumption in \eqref{eq:M_g} is common in the literature when $g_i$, $i\in [m]$, are nonsmooth functions. If $g_i$, $i\in [m]$, are Lipschitz smooth then their gradients are bounded due to the compactness of $X$. Hence \eqref{eq:M_g} is not a strong assumption for the given setting. Also note that due to definition of subgradient for convex function defined in Section \ref{sec:notation}, we have $\gnorm{g'_i(\cdot)}{}{}\leq M_{g_i}$ which implies $\gnorm{g'_i(y)^\top (x-y)}{}{}\leq \gnorm{g'_i(y)}{}{}\gnorm{x-y}{}{}\leq M_{g_i} \gnorm{x-y}{}{}$. Therefore, using the relations in \eqref{eq:sonstraint-smooth-nonsmooth} and \eqref{eq:M_g}, one can state the following assumption for $g = [g_i,\cdots,g_m]^\top$ and $\chi =  [\chi_i,\cdots,\chi_m]^\top$.
 \begin{subequations}\label{eq:M_g_1}
 	\begin{equation}
 		\gnorm{g(x)-g(y)}{}{}\leq M_{g}\gnorm{x-y}{}{} \quad \forall x,y\in X,
 	\end{equation}
 	\begin{equation}
 		\gnorm{\chi(x)-\chi(y)}{}{}\leq M_{\chi}\gnorm{x-y}{}{} \quad \forall x,y\in X,
 	\end{equation}
 \begin{equation}\label{eq:sonstraint-smooth-nonsmooth-1}
 	\gnorm{g(x)-g(y) - \inner{g'(y)}{x-y}}{}{} \le \tfrac{L_{g}}{2}\gnorm{x-y}{}{2} + H_{g}\gnorm{x-y}{}{}\quad \forall x, y\in X,
 \end{equation}
\begin{equation}
	\gnorm{g'(y)^\top (x-y)}{}{}\leq M_g\gnorm{x-y}{}{}\quad \forall x,y\in X,
\end{equation}
 \end{subequations}
 where $g'(\cdot):=[g'_1(\cdot),\dots, g'_m(\cdot)] \in \mathbb{R}^{n\times  m}$, $M_g  := (\sum_{i=1}^{m}M_{g_i}^2)^{1/2}\text{, }M_{\chi} := (\sum_{i=1}^{m}M_{\chi_i}^2)^{1/2} $, $L_g  := (\sum_{i=1}^{m}L_{g_i}^2)^{1/2}$ and $H_g  := (\sum_{i=1}^{m}M_{H_i}^2)^{1/2}$. We denote $\mu_f$ as the modulus of strong convexity for $f$. We say that the convex problem \eqref{eq:prima-problem} is a smooth composite if \eqref{eq:smooth-nonsmooth} and \eqref{eq:sonstraint-smooth-nonsmooth} are satisfied with $H_f = H_{g_i} = 0$, $\forall i \in [m]$. Otherwise, the problem \eqref{eq:prima-problem} is nonsmooth. In short, \eqref{eq:prima-problem} is composite smooth if $H_f = H_{g_i} = 0$, $\forall i \in [m]$, otherwise it is a nonsmooth problem.In addition in this paper, we denote $\ell_g(x_{t+1},\hat{x}_t)$ a linear approximation of $g(\cdot)$ at point $\hat{x}_t$ with 
 \begin{equation}\label{eq:ell_g}
 	 \ell_g(x_{t+1},\hat{x}_t) : =  g(\hat{x}_t)+\inner{g'(\hat{x}_t)}{x_{t+1}-\hat{x}_t}.
 \end{equation}

 For ease of notation we denote $\ell_g(x_{t+1})$ as $ \ell_g(x_{t+1},\hat{x}_t) $. Now, we are ready to introduce the augmented constraint extrapolation (\aconex) for a \eqref{eq:prima-problem} with stochastic objective function. First, note that the objective function $f$ is evaluated by an stochastic oracle $\mathfrak{F}$ at point $\hat{x}_k$ and $\xi_k$. Second, note that updates for $\wh{x}_{k+1}, \wt{y}_{k+1}$ and $\wb{y}_{k+1}$ are quite simple to compute. It is, however, unclear at this point, how to get $(s_{k+1},x_{k+1})$ satisfying \eqref{eq:conceptual-x-s-update}. Later, we will show an efficient subroutine of getting $(s_{k+1},x_{k+1})$ where we do not need any new $\mathfrak{F}, g'$ or $g$ evaluations, we only perform simple projections onto set $X$ and yet we achieve linear convergence to the required $(s_{k+1},x_{k+1})$.
 \vspace{-6pt}
\begin{algorithm}[H]
	\caption{\textbf{Aug}mented \textbf{Con}straint \textbf{Ex}trapolation method (\aconex)}\label{alg:augConEx}
	\begin{algorithmic}[1]
		\State {\bf Input:} $x_1 \in X$, $y_1$, $\{\rho_{1},\tau_1,L_1\}$, $K$
		\State Set $\wh{x}_1 \gets x_1$, $\wt{y}_1 \gets y_1$, $V_1 \gets g(x_1)+ \chi(x_1)$
		\For{k = $1, \dots, K-1$}
		\State Update $(s_{k+1},x_{k+1})$ satisfying
		\begin{equation}\label{eq:conceptual-x-s-update}
			\begin{split}
				&s_{k+1} \gets\argmin_{s \le \mathbf{0}} \inprod{-\wt{y}_k}{s} + \tfrac{\rho_k}{2}\gnorm{\ell_g(x_{k+1})+ \chi(x_{k+1}) - (1-\tau_k)V_k -s}{}{2},\\
				&x_{k+1} \gets \prox(y_{k+1},\mathfrak{F}(\hat{x}_k,\xi_k) +  g'(\wh{x}_k) y_{k+1},\hat{x}_k,L_k ),\\
			\end{split}
		\end{equation}
		 \begin{equation}\label{eq:Denotes}
			\textbf{Denote: }=\begin{cases}
		 	V_{k+1} \gets& g(x_{k+1})+ \chi(x_{k+1}) - s_{k+1},\\
		 	 \wt{V}_{k+1} \gets& \ell_g(x_{k+1})+ \chi(x_{k+1}) - s_{k+1},\\
		 	 y_{k+1}\gets& \wt{y}_k + \rho_k(\wt{V}_{k+1}-(1-\tau_{k})V_k),\\
		 	\wt{y}_{k+1} \gets& \wt{y}_k + \eta_k[\wt{V}_{k+1} - (1-\tau_k)V_k],\\
		 	\wb{y}_{k+1} \gets& (1-\tau_k)\wb{y}_k + \tau_k y_{k+1},\\
		 	\wh{x}_{k+1} \gets& x_{k+1} + \beta_{k+1}(x_{k+1}-x_k).\\
		 \end{cases}
		 \end{equation}
		\EndFor\\
		\Return $x_K$.
	\end{algorithmic}
\end{algorithm} 
\subsection{One-iteration analysis}
Notice from optimality of $s_{k+1}$ and the definition of $y_{k+1}$ based on \eqref{eq:Denotes} of Algorithm \ref{alg:augConEx}, one can say $y_{k+1}= -\grad h(s_{k+1})$ where
\[
h(s): = \inprod{-\wt{y}_k}{s} + \tfrac{\rho_k}{2}\gnorm{\ell_g(x_{k+1})+ \chi(x_{k+1}) - (1-\tau_k)V_k -s}{}{2}.
\]
Moreover, since $\grad h(s_{k+1})  + N_{\{s:s\leq \mathbf{0}\}}(s_{k+1})\ni \mathbf{0} $, one can conclude that $y_{k+1}\in  N_{\{s:s\leq \mathbf{0}\}}(s_{k+1})$ meaning $y_{k+1}\geq \mathbf{0}$. 
Now, we are ready to mention the following lemma. 
	\begin{lemma}\label{lemma:importantlemma}
	Suppose $\tfrac{\eta_k}{2} \le \rho_k$ and $L_k\geq 2L_f+2BL_g$, where $B\geq 0$. Then for all $(x,s,y)\in X\times \mathbb{R}_{-}^m\times\mathbb{R}_{+}^m$ and $k=1,\dots, K-1$, we have
	\begin{align*}
		\Lcal(x_{k+1}, &s_{k+1}, y) - \Lcal(x,s,\wb{y}_{k+1}) - (1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)] \\
		&\le\tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2} -\tau_k\inner{\delta_k }{\dot{x}_k-x} \nonumber\\
		&\quad + \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} ] + \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}- \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2.  
	\end{align*}
where $\ell_g(x_{k+1}) $ is defined as \eqref{eq:ell_g}, $\delta_k = f'(\hat{x}_k) - \mathfrak{F}(\hat{x}_k,\xi_k)$ and $\dot{x}_k = \tfrac{\hat{x}_k-(1-\tau_{k})x_k}{\tau_k}$. 
\end{lemma}
	\begin{proof}
	First, using optimality of $x_{k+1}$, we have for all $x\in X$
	\begin{equation}\label{eq:int_rel2}
		\begin{aligned}
			\inprod{f'(\wh{x}_k) + g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x}&+ \inner{\delta_k }{\hat{x}_k-x} + \chi_0(x_{k+1}) - \chi_0(x) + \inner{\chi(x_{k+1})-\chi(x))}{y_{k+1}} \\
			& \le \tfrac{L_k}{2} [\gnorm{x-\wh{x}_k}{}{2} - \gnorm{x-x_{k+1}}{}{2} - \gnorm{x_{k+1}-\wh{x}_k}{}{2}]+\inner{\delta_k}{\hat{x}_k-x_{k+1}}.
		\end{aligned}
	\end{equation}
	Using strong-convexity and convexity of $f, g$ respectively, Lipschitz property of $f$ and definition of $\ell_g(x_{k+1})$, we have for all $x\in X$
	\begin{align*}
		f(x_{k+1}) &\le f(\wh{x}_k) + \inprod{f'(\wh{x}_k)}{x_{k+1}-\wh{x}_k} + \tfrac{L_f}{2}\gnorm{x_{k+1}-\wh{x}_k}{}{2} + H_f\gnorm{x_{k+1}-\wh{x}_k}{}{},\\
		f(\wh{x}_k) &\le f(x) + \inprod{f'(\wh{x}_k)}{\wh{x}_k-x}- \tfrac{\mu_f\|x-\hat{x}_k\|^2}{2},\\
		g(\wh{x}_k) &\le g(x) + \inprod{g'(\wh{x}_k)}{\wh{x}_k-x},\\
		\ell_g(x_{k+1})&= g(\wh{x}_k) + \inprod{g'(\wh{x}_k)}{x_{k+1}-\wh{x}_k}.
		% \inprod{f'(\wh{x}_k) + g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x}
		% &= \inprod{f'(\wh{x}_k) }{x_{k+1}-\wh{x}_k+ \wh{x}_k - x} + \inprod{g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x} 
		% \ge f(x_{k+1})-f(\wh{x}_k) - \tfrac{L_f}{2}\gnorm{x_{k+1}-\wh{x}_k}{}{2} - H_f\gnorm{x_{k+1}-\wh{x}_k}{}{} + f(x)
	\end{align*}
	Multiplying the last two relations by $y_{k+1}$, noting that $y_{k+1} \ge \mathbf{0}$ and then summing the above relations, we have for all $x \in X$
	\begin{align*}
		f(x_{k+1}) -f(x) &+ \inprod{y_{k+1}}{\ell_g(x_{k+1}) - g(x)}-  \tfrac{L_f}{2}\gnorm{x_{k+1}-\wh{x}_k}{}{2} - H_f\gnorm{x_{k+1}-\wh{x}_k}{}{} + \tfrac{\mu_f\|x-\hat{x}_k\|^2}{2} \\
		&\le \inprod{f'(\wh{x}_k) + g'(\wh{x}_k)y_{k+1}}{x_{k+1}-x}. 
	\end{align*}
	Using the above relation inside \eqref{eq:int_rel2}, we have for all $x\in X$
	\begin{equation}\label{eq:int_rel4}
		\begin{split}
			f(x_{k+1}) -& f(x) + \inprod{y_{k+1}}{\ell_g(x_{k+1}) -g(x)}+\inner{\delta_k }{\hat{x}_k-x} +\chi_0(x_{k+1}) - \chi_0(x) + \inner{\chi(x_{k+1})-\chi(x))}{y_{k+1}}\\ &\le  \tfrac{(L_k-\mu_f)\gnorm{x-\wh{x}_k}{}{2}}{2}- \tfrac{L_k\gnorm{x-x_{k+1}}{}{2}}{2}
			 - \tfrac{L_k-L_f\gnorm{x_{k+1}-\wh{x}_k}{}{2}}{2} + H_f\gnorm{x_{k+1}-\wh{x}_k}{}{}+\inner{\delta_k}{\hat{x}_k-x_{k+1}}.
		\end{split}
	\end{equation}
	Similarly, using first-order optimality condition of $s_{k+1}$ and noting $y_{k+1}\geq \mathbf{0}$, we have for all $s \le \mathbf{0}$, 
	\begin{equation}\label{eq:int_rel3}
		\inprod{y_{k+1}}{s - s_{k+1}} \le 0.
	\end{equation}
	Also, let us consider these two equations 
	\begin{equation}\label{eq:recurtion}
		\begin{aligned}
			&(1-\tau_k)\|x_{k+1} - x_{k}\|^2 + \tau_k\|x_{k+1}-x\|^2 = \|x_{k+1}-(1-\tau_k)x_k-\tau_kx\|^2 + \tau_k(1-\tau_k)\|x_k-x\|^2,\\
			&(1-\tau_k)\|\hat{x}_k - x_{k}\|^2 + \tau_k\|\hat{x}_k-x\|^2 = \|\hat{x}_k-(1-\tau_k)x_k-\tau_kx\|^2 + \tau_k(1-\tau_k)\|x_k-x\|^2,\quad \forall x\in X.
		\end{aligned}
	\end{equation}
	Now, we sum the following four relations: (1) Multiply \eqref{eq:int_rel4} by $\tau_k \in (0,1]$, (2) multiply \eqref{eq:int_rel3} by $\tau_k$, (3) use $x=x_k$ in \eqref{eq:int_rel4} and multiply by $1-\tau_k$, and (4) use $s= s_k$ in \eqref{eq:int_rel3} and multiply by $1-\tau_k$. Then regarding \eqref{eq:recurtion}, we have for all $x \in X, s \le \mathbf{0}$
	\begin{align}
		&f(x_{k+1}) + \chi_0(x_{k+1}) - \tau_k(f(x)+ \chi_0(x)) -(1-\tau_k)(f(x_k)+ \chi_0(x_k))+\inner{\delta_k }{\hat{x}_k-\tau_kx - (1-\tau_k)x_k}\label{eq:int_rel5}\\
		&\quad  + \inprod{y_{k+1}}{\ell_g(x_{k+1})+ \chi(x_{k+1}) - s_{k+1} - \tau_k (g(x)+\chi(x)-s) - (1-\tau_k)(g(x_k)+\chi(x_k)-s_k)}\nonumber\\
		& \le  \tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}\nonumber\\
		&\quad - \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2 - \tfrac{L_k-L_f}{2}\gnorm{x_{k+1} - \wh{x}_k}{}{2} +  H_f\gnorm{x_{k+1}-\wh{x}_k}{}{}+\inner{\delta_k}{\hat{x}_k-x_{k+1}}\nonumber.
	\end{align}
	Finally, noting that $\wt{y}_{k+1} = \argmin_{y} -\inprod{\wt{V}_{k+1} - (1-\tau_k)V_k}{y} + \tfrac{1}{2\eta_k} \gnorm{y-\wt{y}_k}{}{2}$, we have
	\begin{align*}
		\inprod{\wt{V}_{k+1} - (1-\tau_k)V_k}{y-\wt{y}_{k+1}} \le \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} - \gnorm{\wt{y}_{k+1}-\wt{y}_k}{}{2}].
	\end{align*}
	Adding the above relation with \eqref{eq:int_rel5} and noting definitions of $\wt{V}_{k+1}, V_k$ with respect to \eqref{eq:Denotes},  we have
	\begin{equation}\label{eq:int_rel6}
	\begin{aligned}
		&f(x_{k+1}) + \chi_0(x_{k+1}) - \tau_k(f(x)+ \chi_0(x)) -(1-\tau_k)(f(x_k)+ \chi_0(x_k))+\inner{\delta_k }{\hat{x}_k-\tau_kx - (1-\tau_k)x_k}\\
		&\quad-\inprod{\tau_k y_{k+1}}{g(x)+\chi(x)-s} + \inprod{y}{\wt{V}_{k+1} - (1-\tau_k)V_k}\\
		& \le \inprod{\wt{y}_{k+1}-y_{k+1}}{\wt{V}_{k+1} - (1-\tau_k)V_k} - \tfrac{L_k-L_f}{2}\gnorm{x_{k+1} - \wh{x}_k}{}{2} +  H_f\gnorm{x_{k+1}-\wh{x}_k}{}{}\\
		&\quad +\tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}\\
		&\quad + \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} - \gnorm{\wt{y}_{k+1}-\wt{y}_k}{}{2}]+\inner{\delta_k }{\hat{x}_k-x_{k+1}}- \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2.
	\end{aligned}
	\end{equation}
	From the definitions of $y_{k+1}$ and $\wt{y}_{k+1}$ in \eqref{eq:conceptual-x-s-update}and \eqref{eq:Denotes} of Algorithm \ref{alg:augConEx}, we have 
	$\inprod{\wt{y}_{k+1}-y_{k+1}}{\wt{V}_{k+1} - (1-\tau_k)V_k} = (\eta_k-\rho_k) \gnorm{\wt{V}_{k+1} - (1-\tau_k)V_k}{}{2}$. Moreover, $-\tfrac{1}{2\eta_k}\gnorm{\wt{y}_{k+1} - \wt{y}_k}{}{2} = -\tfrac{\eta_k}{2}\gnorm{\wt{V}_{k+1} - (1-\tau_k)V_k}{}{2}$. Using these two relations in \eqref{eq:int_rel6}, alongside with \eqref{eq:conjugate} and Cauchy-Schwarz inequality for $\inner{\delta_k }{\hat{x}_k-x_{k+1}}$ we have 
	\begin{align*}
		&\Lcal(x_{k+1}, s_{k+1}, y) - \Lcal(x,s,\wb{y}_{k+1}) - (1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)] \\
		& \le \tfrac{\eta_k - 2\rho_k}{2}\gnorm{\wt{V}_{k+1} - (1-\tau_k)V_k}{}{2} - \tfrac{L_k-L_f}{2}\gnorm{x_{k+1} - \wh{x}_k}{}{2} +  (H_f+\|\delta_k\|)\gnorm{x_{k+1}-\wh{x}_k}{}{}\nonumber\\
		&\quad +\tfrac{(L_k-\mu_f)\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2} - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}- \tfrac{\mu_f\tau_k(1-\tau_k)}{2}\|x_k-x\|^2 \nonumber\\
		&\quad + \tfrac{1}{2\eta_k}[\gnorm{y-\wt{y}_k}{}{2} - \gnorm{y-\wt{y}_{k+1}}{}{2} ] + \inprod{y}{g(x_{k+1}) - \ell_g(x_{k+1})}-\inner{\delta_k }{\hat{x}_k-\tau_kx - (1-\tau_k)x_k}.
	\end{align*}
	Considering the following relations, one can conclude the proof
	\begin{subequations}
		\begin{equation*}
			(H_f+\|\delta_k\|)\gnorm{x_{k+1}-\wh{x}_k}{}{}\nonumber \leq \tfrac{L_k\gnorm{x_{k+1}-\wh{x}_k}{}{2}\nonumber}{4} + \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k},
		\end{equation*}
		\begin{equation*}
			\begin{aligned}
				\langle y , g(x_{k+1})- \ell_g(x_{k+1})\rangle \leq& \tfrac{L_g}{2}  \| y\| \| x_{k+1}- \hat{x}_k\|^2 + H_g\|y\|\| x_{k+1}- \hat{x}_k\|, \\
				& = \tfrac{L_g}{2} (\| y\| - B)\| x_{k+1}- \hat{x}_k\|^2 + \tfrac{B L_g}{2}\| x_{k+1} - \hat{x}_k\|^2 + H_g\|y\|\| x_{k+1}- \hat{x}_k\|,\\
				& \leq (L_gD_x [\| y\| - B]_++H_g\|y\|) \| x_{k+1}- \hat{x}_k\| + \tfrac{B L_g}{2}\| x_{k+1} - \hat{x}_k\|^2,
			\end{aligned}
		\end{equation*}
		\begin{equation*}
		(L_gD_x  [\| y\| - B]_++H_g\|y\|) \| x_{k+1}- x_k\| - \tfrac{L_k-2(L_f + BL_g)}{4} \| x_{k+1}- \hat{x}_k\|^2\leq \tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}.
	\end{equation*}
	\end{subequations}
\end{proof}
\subsection{Computation of the implicit update in \aconex}
Now, we show a computational scheme for evaluating the update in \eqref{eq:conceptual-x-s-update} in Algorithm \ref{alg:x-s-update} below. We first define the following $ \prox $ operator which is used inside Algorithm \ref{alg:augConEx}.
\begin{equation}\label{eq:prox-operaotr1}
	F(\bx) := \prox \paran[\Big]{\rho_k\bracket[\big]{U_k + g'(\hat{x}_k)^\top \bx  + \chi (\bx)}_+,\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx+\chi (\bx)]_+, \wh{x}_k, L_k}
\end{equation}

where $U_k = g(\wh{x}_k) - g'(\wh{x}_k)^T\wh{x}_k - (1-\tau_k)V_k + \tfrac{\wt{y}_k}{\rho_k}$. Equivalently, one can use the classical definition of $\proximal$ operator and rewrite  $F(\bx)$ in \eqref{eq:prox-operaotr1} as follows 
\begin{equation}\label{eq:prox-operaotr2}
	F(\bx) = \proximal_{\Gamma(x;\bx)/L_k}\paran[\Big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx+\chi (\bx)]_+}},
\end{equation}
where $\Gamma(x;\bx) = I_X(x)+\chi_0(x) + \inner{\chi(x)}{c(\bx)}$, $c(\bx) = \rho_k [U_k + g'(\wh{x}_k)^\top \bx + \chi(\bx)]_+$ and $I_X(x)$ is the indicator function of set $X$. Note that $c(\bx):\mathbb{R}^n\rightarrow \mathbb{R}^m$ is a mapping independent of $x$. 
\begin{algorithm}[H]
	\caption{Compute \eqref{eq:conceptual-x-s-update}}
	\label{alg:x-s-update}
	\begin{algorithmic}
		\State $w_0 = \wh{x}_k$
		\For{ $t = 0, \dots, T-1$}
		\State $w_{t+1} = F(w_t)$
		\EndFor
		\Return $w_T$.
	\end{algorithmic}
\end{algorithm}
The algorithm above tries to compute the fixed point of $F$. In what follows, we show that $x_{k+1}$ is a fixed point of $F$. Moreover, if $L_k$ satisfies a simple condition, then $x_{k+1}$ is a unique fixed point and Algorithm \ref{alg:x-s-update} converges linearly. Before we show this result, we require a technical proposition which we state below first.


\begin{proposition}\label{prop:a-b-relation}
	For vectors $a, b$, we have $\gnorm{[a]_+ - [b]_+}{}{} \le \gnorm{a-b}{}{}$
\end{proposition}
\begin{proof}
	It suffices to prove the following inequality for any two scalars $s_1, s_2$, we have  \[|[s_1]_+-[s_2]_+| \le |s_1-s_2|.\] Indeed, if the above relation holds, applying this elementwise to vectors $a, b$ yields the desired result.
	We divide it into three cases:\\
	{\bf Case 1:} $s_1 \ge 0, s_2 \ge 0$. Then, $|[s_1]_+-[s_2]_+|  = |s_1-s_2|$.\\
	{\bf Case 2:} $s_1 < 0, s_2 < 0$. Then, $|[s_1]_+-[s_2]_+| = 0 \le |s_1-s_2|$.\\
	{\bf Case 3:} Either $s_1 < 0$ or $s_2 < 0$. Without loss of generality, we assume $s_2 < 0$. Then, $|[s_1]_+-[s_2]_+| = s_1 \le |s_1-s_2|$.\\
	In all three cases, we showed the required relation. Hence, we conclude the proof.
\end{proof}
Now, we show that $F$ is a contraction operator when $L_k$ is large enough.
\begin{lemma}\label{lem:F-contraction}
	If $L_k\geq 2\rho_k(M_g + M_{\chi})^2$, then $F$ is a contraction operator satisfying satisfying $\gnorm{F(\bx_1) - F(\bx_2)}{}{} \le \tfrac{1}{2} \gnorm{\bx_1-\bx_2}{}{}$. Moreover, $x_{k+1}$ is the unique fixed point of $F$.
\end{lemma}
\begin{proof}
	Note that 
	\[
	s_{k+1}=[U_k + g'(\wh{x}_k)^\top x_{k+1}+\chi (x_{k+1})]_-.
	\]
	Consequently, from the definition of $y_{k+1}$ in \eqref{eq:Denotes}, one can say 
	\[
	y_{k+1} = [U_k + g'(\wh{x}_k)^\top x_{k+1}+\chi (x_{k+1})]_+.
	\]
	Replacing this value into $x_{k+1}$ update in Algorithm \ref{alg:augConEx} and by equivalency between \eqref{eq:prox-operaotr1} and \eqref{eq:prox-operaotr2}, we have 
	\begin{equation*}
		\begin{aligned}
			x_{k+1}=& \proximal_{\Gamma(x;x_{k+1})/L_k}\paran[\Big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top x_{k+1}+\chi (x_{k+1})]_+}}\\
			=& F(x_{k+1}).
		\end{aligned}
	\end{equation*}
From the above relation, it is clear that $x_{k+1}$ is a fixed point of the operator $F(\bx)$. 
	Next, let us define $\mathcal{T}(\bx)$ such that 
	\[
	\mathcal{T}(\bx) = \wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx+\chi (\bx)]_+},
	\]
	Also suppose $\mathcal{T}_1= \mathcal{T}(\bx_1),\mathcal{T}_2= \mathcal{T}(\bx_2)$ and let $u_1 = F(\bx_1), u_2 = F(\bx_2)$. Then, one can construct the following relations
	\begin{subequations}
		\begin{equation*}
			\partial\tfrac{\chi_0(u_1)}{L_k }+ \partial\tfrac{\chi(u_1)}{L_k}^\top c(\bx_1) + u_1-\mathcal{T}_1 \ni \mathbf{0}
		\end{equation*}
		\begin{equation*}
			\partial\tfrac{\chi_0(u_2)}{L_k }+ \partial\tfrac{\chi(u_2)}{L_k}^\top c(\bx_2) + u_2-\mathcal{T}_2 \ni \mathbf{0}
		\end{equation*}
	\end{subequations}
	Consequently, 
	\begin{subequations}
		\begin{equation*}
			\partial_{\tfrac{\chi_0+\chi^\top c(\bx_1)}{L_k}} (u_1) \in \mathcal{T}_1-u_1
		\end{equation*}
		\begin{equation*}
		\partial_{\tfrac{\chi_0+\chi^\top c(\bx_1)}{L_k}} (u_2) \in \mathcal{T}_2-u_2 - \tfrac{\chi'(u_2)}{L_k}^\top(c(\bx_2)-c(\bx_1)),
		\end{equation*}
	\end{subequations}
	where $\tfrac{\chi'(u_2)}{L_k}$ is a subgradient in $\partial \tfrac{\chi(u_2)}{L_k}$.  Using the fact that $\Gamma(\cdot;\bx_1)/L_k$ is a convex function, then $\partial_{\tfrac{\chi_0+\chi^\top c(\bx_1)}{L_k}}$ is a monotone operator, we have 
	\begin{equation*}
		\inner{\mathcal{T}_1-u_1-\mathcal{T}_2+u_2 +  \tfrac{\chi'(u_2)}{L_k}^\top(c(\bx_2)-c(\bx_1))}{u_1-u_2}\geq 0
	\end{equation*}
Hence one can conclude the following inequality
\[
\inner{\mathcal{T}_1-\mathcal{T}_2}{u_1-u_2} + \inner{\tfrac{\chi'(u_2)}{L_k}^\top(c(\bx_2)-c(\bx_1))}{u_1-u_2}\geq \|u_1-u_2\|^2
\]
By Cauchy-Schwarz inequality, assumptions in \eqref{eq:M_g_1} and definition of $c(\bx)$ in \eqref{eq:prox-operaotr2}, one can write the following 
\begin{equation}\label{eq:proj_1}
	\gnorm{\mathcal{T}_1-\mathcal{T}_2}{}{} + \tfrac{\rho_k M_\chi(M_g+M_\chi)}{L_k}\gnorm{\bx_1-\bx_2}{}{}\geq \|u_1-u_2\|
\end{equation}
Moreover, from the definition of $\mathcal{T}(\bx)$, one can have the following relations for $\gnorm{\mathcal{T}_1-\mathcal{T}_2}{}{}$ 
\begin{equation}\label{eq:proj2}
	\begin{aligned}
		\gnorm{\mathcal{T}_1-\mathcal{T}_2}{}{}& = \big\|  \bracket[\big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx_1+\chi (\bx_1)]_+}} \\
		&\qquad - \bracket[\big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx_2+\chi (\bx_2)]_+}} \big\|\\
		&= \tfrac{\rho_k}{L_k} \gnorm{g'(\wh{x}_k)\braces{[U_k + g'(\wh{x}_k)^T\bx_2 + \chi(\bx_2)]_+ - [U_k + g'(\wh{x}_k)^T\bx_1+\chi(\bx_1)]_+} }{}{}\\
		&\le \tfrac{\rho_kM_g}{L_k} \gnorm{[U_k + g'(\wh{x}_k)^T\bx_2 + \chi(\bx_2)]_+ - [U_k + g'(\wh{x}_k)^T\bx_1+\chi(\bx_1)]_+}{}{}\\
		&\le \tfrac{\rho_kM_g}{L_k} \gnorm{g'(\wh{x}_k)^T(\bx_2-\bx_1) + \chi(\bx_2)-\chi(\bx_1)}{}{}\\
		&\le \tfrac{\rho_kM_g (M_g + M_\chi)}{L_k} \gnorm{\bx_1-\bx_2}{}{},
	\end{aligned}
\end{equation}
where  the first and third inequalities follow by Assumptions in \eqref{eq:M_g_1}, and second inequality follows by Proposition \ref{prop:a-b-relation}. Therefore, using \eqref{eq:proj_1} and \eqref{eq:proj2}, we have
\[
\gnorm{u_1-u_2}{}{}\leq \tfrac{\rho_k(M_g+M_\chi)^2}{L_k}\gnorm{\bx_1-\bx_2}{}{}.
\]
Taking $L_k\geq 2\rho_k(M_g + M_{\chi})^2$ becomes $F$ a contraction, we note that $x_{k+1}$ is unique fixed point \cite{blah}.
Hence, we conclude the proof. 
\end{proof}
\iffalse
\begin{lemma}\label{lem:F-contraction}
	If $L_k \ge 2\rho_kM_g(M_g+ M_\chi) (1+\rho_kM_\chi^2 + \rho_kM_\chi M_g)$, then $F$ is contraction operator satisfying $\gnorm{F(\bx_1) - F(\bx_2)}{}{} \le \tfrac{1}{2} \gnorm{\bx_1-\bx_2}{}{}$. Moreover, $x_{k+1}$ is the unique fixed point of $F$.
\end{lemma}
\begin{proof}
	Note that 
	\begin{equation}\label{eq:int_rel7}
		s_{k+1} = \bracket[\big]{\underbracket{g(\wh{x}_k) - g'(\wh{x}_k)^T\wh{x}_k - (1-\tau_k)V_k + \tfrac{\wt{y}_k}{\rho_k}}_{U_k}+ g'(\wh{x}_k)^Tx_{k+1}+\chi(x_{k+1})}_-.
	\end{equation}
	Replacing this value into $x_{k+1}$ update, we have
	\begin{align*}
		x_{k+1} &= \proximal_{\Gamma(x)}\bracket[\Big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^Tx_{k+1}+\chi(x_{k+1}) -s_{k+1}]}}\\
		&= \proximal_{\Gamma(x)}\bracket[\Big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^Tx_{k+1}+\chi(x_{k+1})]_+}}\\
		&= F(x_{k+1}),
	\end{align*}
	where the first relation uses the definition of $U_k$, and second relation uses \eqref{eq:int_rel7}.
	From the above relation, it is clear that $x_{k+1}$ is a fixed point of the operator $F(\bx)$.
	
	%We show that under appropriate condition on $L_k$, the operator $F(\bx)$ is a contraction and hence, the iteration scheme $\{\bw_{t+1} = F(\bw_t)\}_{t=0}^T$ converges linearly to $x_{k+1}$.
	
	Note that from \eqref{eq:proximal-proof} we have the following 
	\[
		F(\bt) := \proximal_{\Gamma(x)}\paran{\bt},
	\] . Hence, from Proposition \ref{prop:firmly-non-expansive} and the following relation
	\[
	\bt = \wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx+\chi (\bx)]_+},
	\]
	we have
	\begin{align*}
		\gnorm{F(\bt_1) - F(\bt_2)}{}{}
		&= \big\| \proximal_{\Gamma(x)} \bracket[\big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx_1+\chi (\bx_1)]_+}} \\
		&\qquad - \proximal_{\Gamma(x)} \bracket[\big]{\wh{x}_k - \tfrac{1}{L_k}\braces[\big]{\mathfrak{F}(\wh{x}_k,\xi_k) + \rho_k g'(\wh{x}_k)[U_k + g'(\wh{x}_k)^\top \bx_2+\chi (\bx_2)]_+}} \big\|\\
		&\le \tfrac{(1+\rho_kM_\chi^2 + \rho_kM_\chi M_g)\rho_k}{L_k} \gnorm{g'(\wh{x}_k)\braces{[U_k + g'(\wh{x}_k)^T\bx_2 + \chi(\bx_2)]_+ - [U_k + g'(\wh{x}_k)^T\bx_1+\chi(\bx_1)]_+} }{}{}\\
		&\le \tfrac{(1+\rho_kM_\chi^2 + \rho_kM_\chi M_g)\rho_kM_g}{L_k} \gnorm{[U_k + g'(\wh{x}_k)^T\bx_2 + \chi(\bx_2)]_+ - [U_k + g'(\wh{x}_k)^T\bx_1+\chi(\bx_1)]_+}{}{}\\
		&\le \tfrac{(1+\rho_kM_\chi^2 + \rho_kM_\chi M_g)\rho_kM_g}{L_k} \gnorm{g'(\wh{x}_k)^T(\bx_2-\bx_1) + \chi(\bx_2)-\chi(\bx_1)}{}{}\\
		&\le \tfrac{(1+\rho_kM_\chi^2 + \rho_kM_\chi M_g)\rho_kM_g (M_g + M_\chi)}{L_k} \gnorm{\bx_1-\bx_2}{}{} \le \tfrac{1}{2}\gnorm{\bx_1-\bx_2}{}{},
	\end{align*}
	where the first inequality follows by Proposition \ref{prop:firmly-non-expansive}, second and fourth inequality follows by $\gnorm{g'(x)}{}{} \le M_g$ for all $x \in X$, and third inequality follows by Proposition \ref{prop:a-b-relation}. Since $F$ is a contraction, we note that $x_{k+1}$ is unique fixed point \cite{blah}.
	Hence, we conclude the proof. 
\end{proof}
\fi
	\begin{theorem}
	Let $\{w_t\}_{t=1}^T$ be the sequence generated by Algorithm \ref{alg:x-s-update}. If conditions in Lemma \ref{lem:F-contraction} are satisfied then 
	$\gnorm {w_T-x_{k+1}}{}{} \le2^{-T}\gnorm{\wh{x}_k - x_{k+1}}{}{}.$ Furthermore, implementing Algorithm \ref{alg:x-s-update} requires only $T$ projections onto set $X$.
\end{theorem}
\begin{proof}
	Note that 
	\begin{align*}
		\gnorm{w_{t+1} - x_{k+1}}{}{} &= \gnorm{F(w_t) - x_{k+1}}{}{}\\
		&= \gnorm{F(w_t) - F(x_{k+1})}{}{}\\
		&\le \tfrac{1}{2} \gnorm{w_t - x_{k+1}}{}{},
	\end{align*}
	where first equality follows by definition of $w_{t+1}$, second equality uses the fact that $x_{k+1}$ is a fixed point of $F$, and final inequality uses contraction property from Lemma \ref{lem:F-contraction}. Exapnding the above recursion, we obtain
	\[ \gnorm{w_{T} - x_{k+1}}{}{} \le 2^{-T}\gnorm{w_0 - x_{k+1}}{}{} =  2^{-T}\gnorm{\wh{x}_k - x_{k+1}}{}{},\]
	where the last relation uses $w_0 = \wh{x}_k$ as stated in Algorithm \ref{alg:x-s-update}. It is also clear each iteration of Algorithm \ref{alg:x-s-update} requires computing $F(w_t)$ only. Hence, we conclude the proof.
\end{proof}

\begin{remark}
	Note that Algorithm \ref{alg:x-s-update} does not need any new computation of $\mathfrak{F}, g$ or $g'$. Hence, the gradient complexity of Algorithm \ref{alg:augConEx} exactly equals $K$ even though it requires additional proximal operations in the inner loop. Since $X$ is an easy set to project onto, and we have linear convergence, we can get arbitrarily close to $x_{k+1}$ very fast with not much computational effort. Moreover, as the algorithm proceeds, the last iterate $x_k$ is supposed get close to $x^*$. Hence, distance between $\wh{x}_k$ and $x_{k+1}$ will decrease as well. Hence, there is a warm-starting effect of choosing $w_0 = \wh{x}_k$.
\end{remark}

In view of fast converging and computationally cheap method for update \eqref{eq:conceptual-x-s-update}, we henceforth assume that it can be computed directly henceforth.

\subsection{Convergence analysis for the convex problem}
\begin{theorem}\label{thm:convex-case}
	Suppose the conditions in \eqref{eq:smooth-nonsmooth} and \eqref{eq:M_g_1} are satisfied for the convex problem in \eqref{eq:prima-problem} with $\mu_f = 0$. Let $B\geq 1$ be a constant. Set $K\geq 2$ and assume $\{\rho_{k},\tau_k,L_k,\beta_{k+1}\}_{k\geq 1}$ are generated by the following step-size policy parameter in Algorithm \ref{alg:augConEx}
		\begin{equation}\label{eq:non-ergo-stepsize-non-smooth-eta}
		\begin{aligned}
			&\tau_k = \tfrac{2}{k+1}, \quad \rho_{k+1} = \rho_1 (2+k),\quad
			\eta_k = \rho_{1}\tfrac{k^2}{K},\quad
			\beta_{k+1} = \tfrac{(1-\tau_{k})\tau_{k+1}}{\tau_{k}}\\
			& L_k =L=  2(L_f+ BL_g + \rho_{1}K(M_g + M_\chi)^2)+\tfrac{K\sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+\sigma^2))}}{120D_X},
		\end{aligned}
	\end{equation}
	where $\mathcal{H}_*=(L_gD_x  [\| y^\ast\|+1 - B]_++H_g(\|y^\ast\|+1) )$. Then, we have the following bounds for optimality and feasibility gaps 
 \begin{equation*}
 	\begin{aligned}
 		\Ebb[\psi_0(x_K)- \psi_0(x^*)]\leq&\tfrac{D_X\sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+ \sigma^2))}}{6(K-1)}+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 \|^2 + \tfrac{40D_X^2(L_f+ BL_g +\rho_{1} K(M_g + M_\chi)^2)}{(K-1)K}\\
 		& \quad+\tfrac{80D_X(K+3)(H_f^2+ \sigma^2)}{K(240D_X\rho_{1}(M_g+M_\chi)^2 + \sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+\sigma^2))})}+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}.
 	\end{aligned}
 \end{equation*}
	and 
	\begin{equation*}
		\begin{aligned}
			\Ebb(\|[\psi(x_K)]_+\|)& \leq  \tfrac{D_X\sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+ \sigma^2))}}{6(K-1)} + \tfrac{40D_X^2(L_f+ BL_g + K(M_g + M_\chi)^2)}{(K-1)K}\\
			& \quad + \tfrac{80D_X(K+3)(8(H_f^2+ \sigma^2) +\mathcal{H}_*^2 )}{K(240D_X\rho_{1}(M_g+M_\chi)^2 + \sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+\sigma^2))})}+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 - \hat{y} \|^2 \\
			&\quad +\tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}
		\end{aligned}
	\end{equation*} 
\end{theorem}
\begin{proof}
		First, assume the following conditions for the convex problem
	\begin{equation}\label{eq:conditions}
		\tfrac{\eta_k}{2}\leq \rho_k, \quad L_k\geq 2(L_f+ BL_g + \rho_k(M_g+M_\chi)^2),\quad \tfrac{1}{\eta_k}\leq \tfrac{1-\tau_k}{\eta_{k-1}}.
	\end{equation}
	Thus, one can easily varefiy that the step-size policy in \eqref{eq:non-ergo-stepsize-non-smooth-eta} satisfies the conditions in \eqref{eq:conditions} for $k\geq 2$. 
	Second, letting $\tilde{x}_k  = \tfrac{1}{\tau_k}[\hat{x}_k-(1-\tau_k)x_k]$ and $\tilde{x}_{k+1}  = \tfrac{1}{\tau_k}[x_{k+1}-(1-\tau_k)x_k]$, and taking the expectation from both sides regarding \eqref{eq:SO_F_objective}, we can write the following recursion for $k\geq 2$
	\begin{equation}\label{eq:non-ergo-5-non-smooth-recur-eta}
		\begin{aligned}
			&\Ebb[\Lcal(x_{k+1},s_{k+1}, y)- \Lcal(x,s,\bar{y}_{k+1})  + \tfrac{1}{2\eta_k}\|\tilde{y}_{k+1}-y\|^2]\leq \Ebb\big[
			(1-\tau_k)[ \Lcal(x_{k},s_{k}, y)- \Lcal(x,s,\bar{y}_{k})
			+  \tfrac{1}{2\eta_{k-1}}\|\tilde{y}_k-y\|^2\big]\\
			&+\Ebb\big[\tfrac{\tau_k^2L_k}{2}[\|\tilde{x}_k-x\|^2- \|\tilde{x}_{k+1}-x\|^2]\big] -\tau_k\Ebb[\inner{\delta_k }{\dot{x}_k-x}]
			+ \Ebb\big[ \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}\big]+ \tfrac{2(H_f^2+ \sigma^2)}{L_k}.
		\end{aligned}
	\end{equation}
	Consequently, one can write the following recursion 
	\begin{equation}\label{eq:recur-nonsmooth-eta}
		\begin{aligned}
			&\Ebb[\Lcal(x_{K},s_{K}, y)- \Lcal(x,s,\bar{y}_{K})] \leq  [\prod_{k=2}^{K-1}(1-\tau_k)]\Ebb[\Lcal(x_{2},s_{2}, y)- \Lcal(x,s,\bar{y}_{2})+ \tfrac{1}{2\eta_{1}}\|\tilde{y}_2-y\|^2]\\
			& \quad  +\Ebb\big[ \sum_{k=2}^{K-1} [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tfrac{\tau_k^2L_k}{2}[\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big] -\Ebb\big[\sum_{k=2}^{K-1}[\prod_{i=k+1}^{K-1}(1-\tau_{i})]\tau_k\inner{\delta_k}{\dot{x}_k-x}\big] \\
			& \quad + \sum_{k=2}^{K-1}\big[[ \prod_{i=k+1}^{K-1} (1-\tau_{i})] \Ebb\big[ \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}\big] + \tfrac{2(H_f^2+ \sigma^2)}{L_k}\big].
		\end{aligned}
	\end{equation}
	Now, let us simplify each line in the RHS of \eqref{eq:recur-nonsmooth-eta}. Note that from Lemma \ref{lemma:importantlemma} and $L_1 = L, \eta_{1} = \tfrac{\rho_{1}}{K}, \hat{x}_1 = x_1 , \tilde{y}_1 = y_1, \tau_1=1$ , we have 
	\begin{equation*}
		\begin{aligned}
			\Ebb&[\Lcal(x_{2},s_{2}, y)-\Lcal(x,s,\bar{y}_{2})+ \tfrac{1}{2\eta_{1}}\|\tilde{y}_2-y\|^2]\leq (1-\tau_1)\Ebb[(\Lcal(x_{1},s_{1}, y)- \Lcal(x,s,\bar{y}_{1}))]\\
			& \quad + 2D_X^2 + \tfrac{K}{2\rho_{1}}\Ebb[\|y_1 - y\|^2] + \Ebb\big[\tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{8\rho_1K(M_g + M_\chi)^2}\big] + \tfrac{H_f^2 + \sigma^2}{\rho_1K(M_g + M_\chi)^2} - \Ebb[\inner{\delta_1}{\dot{x}_1-x}].
		\end{aligned}
	\end{equation*}
	Noting that $\tau_1 = 1$ and $\prod_{k=2}^{K-1}(1-\tau_k) = \tfrac{2}{K(K-1)}$ we have the following relation for the first line in RHS of \eqref{eq:recur-nonsmooth-eta}
	\begin{equation}\label{eq:first summation}
		\begin{aligned}
			[\prod_{k=2}^{K-1}(1-\tau_k)]&\Ebb[\Lcal(x_{2},s_{2}, y)- \Lcal(x,s,\bar{y}_{2})+ \tfrac{1}{2\eta_{1}}\|\tilde{y}_2-y\|^2]\leq \tfrac{4LD_X^2}{K(K-1)} + \tfrac{1}{(K-1)\rho_1}\Ebb[\|y_1 - y\|^2]\\
			&\quad +\Ebb\big[\tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4K^2(K-1)\rho_1(M_g + M_\chi)^2}\big]+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2} - \tfrac{2\Ebb[\inner{\delta_1}{\dot{x}_1-x}]}{K(K-1)},
		\end{aligned}
	\end{equation}
	For the first summation  in the second line of \eqref{eq:recur-nonsmooth-eta} we have 
	\begin{equation}\label{eq:second summation}
		\begin{aligned}
			\Ebb\big(\sum_{k=2}^{K-2}& [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tfrac{\tau_k^2L_k}{2}[\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big) +\Ebb\bracket[\big]{\tfrac{\tau_{K-1}^2L_{K-1}}{2}[\|\tilde{x}_{K-1}-x\|^2-\|\tilde{x}_{K}-x\|^2]}\\
			&  \leq \Ebb\big( \sum_{k=2}^{K-2} \tfrac{ k (k+1)}{(K-1)K} \tfrac{4}{(k+1)^2} \tfrac{ L}{2}[\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big) + \tfrac{4D_X^2L}{K^2} \\
			& = \Ebb\big(\sum_{k=2}^{K-2} \tfrac{2 k }{(K-1)K (k+1)} L [\|\tilde{x}_k-x\|^2-\|\tilde{x}_{k+1}-x\|^2]\big) + \tfrac{4D_X^2L}{K^2}\\
			& = \tfrac{2L}{(K-1)K}\Ebb \Big(\big(\sum_{k=2}^{K-2} \big[\tfrac{k+1}{k+2}
			 -\tfrac{k}{k+1}\big] \|\tilde{x}_{k+1}-x\|^2 \big)+ \tfrac{1}{2}  \|\tilde{x}_{1}-x\|^2\Big) + \tfrac{4D_X^2L}{K^2} \\
			&  = \tfrac{2L}{(K-1)K} \sum_{k=2}^{K-2} \big(\tfrac{k+1}{k+2} - \tfrac{k}{k+1}\big) \Ebb(\|\tilde{x}_{k+1}-x\|^2)  + \tfrac{L}{(K-1)K}  \|\tilde{x}_{1}-x\|^2 + \tfrac{4D_X^2L}{K^2}\\
			& \leq  \tfrac{8L}{(K-1)K} D_x^2 + \tfrac{4L}{(K-1)K} D_x^2 + \tfrac{4L}{K^2}D_X^2\leq  \tfrac{16L}{(K-1)K}D_X^2
		\end{aligned}
	\end{equation}
	The last summation line in the RHS of \eqref{eq:recur-nonsmooth-eta} has the following upper bound.
	\begin{equation}\label{eq:third summation}
		\begin{aligned}
			&\sum_{k=2}^{K-2}\big[[ \prod_{i=k+1}^{K-1} (1-\tau_{i})] \Ebb\big[ \tfrac{(L_gD_x[\|y\|-B]_++ H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}\big] + \tfrac{2(H_f^2+ \sigma^2)}{L_k}\big] + \big[\Ebb[\tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4(L_{K-1}-2(L_f+ BL_g ))}] + \tfrac{2(H_f^2+ \sigma^2)}{L_{K-1}}\big]\\
			& = \Big(\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(K-1)K(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{(K-1)KL}\Big) \sum_{k=2}^{K-2} k(k+1)  + \big[\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{L}\big]\\
			&  \leq \Big(\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(K-1)K(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{(K-1)KL}\Big) \tfrac{ (K-1)^3}{3} + \big[\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \sigma^2)}{L}\big] \\
			& \leq  \tfrac{K\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{12(L-2(L_f+ BL_g ))} +\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} +  \tfrac{2K(H_f^2+ \sigma^2)}{3L}+ \tfrac{2(H_f^2+ \sigma^2)}{L}
		\end{aligned}
	\end{equation} 
	
	Thus from \eqref{eq:first summation}, \eqref{eq:second summation}, and \eqref{eq:third summation}, the recursion in \eqref{eq:recur-nonsmooth-eta} can be written as follows 
	\begin{equation}\label{eq:recur-nonsmooth-eta-4}
		\begin{aligned}
			&\Ebb(\Lcal(x_{K},s_{K}, y)- \Lcal(x,s,\bar{y}_{K})) \leq  \tfrac{20L}{(K-1)K}D_X^2 + \tfrac{1}{(K-1)\rho_{1}}\Ebb[\|y_1 - y\|^2]  + \tfrac{K(8(H_f^2+ \sigma^2) +\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2] )}{12(L-2(L_f+ BL_g ))} \\
			& \quad+ \tfrac{8(H_f^2+ \sigma^2) +\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4(L-2(L_f+ BL_g ))} +\tfrac{\Ebb[(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2]}{4K^2(K-1)\rho_1(M_g + M_\chi)^2}+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}\\
			&-\Ebb\big[\sum_{k=2}^{K-1}[\prod_{i=k+1}^{K-1}(1-\tau_{i})]\tau_k\inner{\delta_k}{\dot{x}_k-x}\big]  - \tfrac{2\Ebb[\inner{\delta_1}{\dot{x}_1-x}]}{K(K-1)}  .
		\end{aligned}
	\end{equation}
	We know that $ \Lcal(x_K,y)\leq \Lcal(x_K,s_K,y)$ and for $s =0$ we have $\Lcal(x,\bar{y}_K) = \Lcal(x,0,\bar{y}_K)$. Therefore, we have the following
	\begin{equation}\label{eq:conjugate-1}
		\Lcal(x_K,y) - \Lcal(x,\bar{y}_K) \leq \Lcal(x_K,s_K,y) - \Lcal(x,0,\bar{y}_K) \quad \forall (x,y)\in X\times \mathbb{R}^m_+.
	\end{equation}
	Now, let us choose $ y =0 $. we know $ \bar{y}_K\geq 0$ and $\psi(x^*)\leq 0$ thus $ \langle \bar{y}_K, \psi(x^*)\rangle \leq 0 $. Also note that $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0$. Therefore, regarding \eqref{eq:recur-nonsmooth-eta-4} and \eqref{eq:conjugate-1}, we have
	\begin{equation*}\label{eq:optimality-gap}
			\Ebb[\psi_0(x_K)- \psi_0(x^*)]\leq\tfrac{		20L}{(K-1)K}D_X^2+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 \|^2 + \tfrac{8(K+3)(H_f^2+ \sigma^2)}{12(L-2(L_f+ BL_g ))}+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2},
	\end{equation*}
 Applying the step-size policy in \eqref{eq:non-ergo-stepsize-non-smooth-eta} we obtain 
 \begin{equation*}
 	\begin{aligned}
 				\Ebb[\psi_0(x_K)- \psi_0(x^*)]\leq&\tfrac{D_X\sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+ \sigma^2))}}{6(K-1)}+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 \|^2 + \tfrac{40D_X^2(L_f+ BL_g +\rho_{1} K(M_g + M_\chi)^2)}{(K-1)K}\\
 				& \quad+\tfrac{80D_X(K+3)(H_f^2+ \sigma^2)}{K(240D_X\rho_{1}(M_g+M_\chi)^2 + \sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+\sigma^2))})}+ \tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}.
 	\end{aligned}
 \end{equation*}
Now, let us move to the feasibility gap. First, observe that 
\begin{equation*}\label{eq:first-frasib}
 	\Lcal(x_K,y^*) - \Lcal(x^*,y^*)\geq 0
\end{equation*}
  
implying that 
\begin{equation*}\label{eq:second-feasib}
	\psi_0(x_K) + \inner{y^*}{\chi(x_K)} - \psi_0(x^*)\geq 0 ,
\end{equation*}

which in the view of below relation 
\begin{equation*}\label{eq:feasib3}
	\inner{y^*}{\psi(x_K)}\leq \inner{y^*}{[\psi(x_K)]_+}\leq \|y^*\|\|[\psi(x_K)]_+\|
\end{equation*}

we have 
\begin{equation}\label{eq:haty}
	\psi_0(x_K) +\|y^*\|\|[\psi(x_K)]_+\| - \psi_0(x^*)\geq 0.
\end{equation}
Moreover, $\Lcal(x_K,\hat{y})-\Lcal(x^*,\bar{y}_K)\geq\Lcal(x_K,\hat{y})-\Lcal(x^*,y^*) = \psi_0(x_K) +(\|y^*\|+1)\|[\psi(x_K)]_+\| - \psi_0(x^*)$. Therefore,  considering \eqref{eq:conjugate-1}, \eqref{eq:haty}, $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0 $, and the definition of $\hat{y}$ as $\hat{y} = (\|y^*\|+1)\tfrac{[g(\bar{x}_K)]_+}{\|[g(\bar{x}_K)]_+\|}$, the feasibility gap can be written as 
	\begin{equation*}
		\begin{aligned}
			\Ebb(\|[\psi(x_K)]_+\|)\leq  \Ebb(\Lcal(x_K,\hat{y})- &\Lcal(x^*,\bar{y}_K)) \leq  \tfrac{D_X\sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+ \sigma^2))}}{6(K-1)} + \tfrac{40D_X^2(L_f+ BL_g + K(M_g + M_\chi)^2)}{(K-1)K}\\
			& \quad + \tfrac{80D_X(K+3)(8(H_f^2+ \sigma^2) +\mathcal{H}_*^2 )}{K(240D_X\rho_{1}(M_g+M_\chi)^2 + \sqrt{120K(\mathcal{H}_*^2 + 8(H_f^2+\sigma^2))})}+ \tfrac{1}{(K-1)\rho_{1}}\|y_1 - \hat{y} \|^2 \\
			&\quad +\tfrac{2(H_f^2 + \sigma^2)}{K^2(K-1)\rho_1(M_g + M_\chi)^2}
		\end{aligned}
	\end{equation*} 
\end{proof} 
Theorem \ref{thm:convex-case} states the convergence result of $\aconex$ method for the stochastic case of optimization problem in \eqref{eq:prima-problem}. One important observation is related to choice of the initial parameter $\rho_{1}$. Specifically, to have the convergence rate of $\mathcal{O}(1/\sqrt{K})$ for the algorithm, one should choose $\rho_{1}$ as $\mathcal{O}(\sqrt{K})$ and $\Omega(1/\sqrt{K})$. In details, one can derive the convergence results for nonsmooth deterministic and stochastic (where we use a stochastic approximation for $f'$). First, let us derive the convergence results for the nonsmooth deterministic case (i.e., $\sigma=0$). Considering $\rho_{1}=1$ the error convergence rate of $\aconex{}$ after $K$ iterations is of 
\[
\mathcal{O}\big( \tfrac{D_X(\mathcal{H}_* + H_f)}{\sqrt{K}} + \tfrac{D_X^2(L_f+BL_g)}{K^2} + \tfrac{D_X^2(M_g+M_\chi)^2}{K}\big)
\]
Assuming $B\geq \|y^*\|+1$, one can assume we have $\mathcal{O}(\tfrac{D_X^2L_g(\|y^*\|+1)}{K^2})$ in terms of $\|\lambda^*\|$ which shows \aconex can effectively balances the effect of $\|\lambda^*\|$. Now, let us consider the stochastic case where $\sigma>0$. We have the following convergence rate of error for $\rho_{1} =1$
\[
\mathcal{O}\big( \tfrac{D_X(\mathcal{H}_* + H_f+\sigma)}{\sqrt{K}} + \tfrac{D_X^2(L_f+BL_g)}{K^2} + \tfrac{D_X^2(M_g+M_\chi)^2}{K}\big)
\]
Observe that the effect of  having stochastic approximation of $f'$ is the same as non-smoothness of $f$. Moreover, assuming $B\geq \|\lambda^*\|+1$, we balance the effect of $\gnorm{\lambda^*}{}{}$ and get similar results as we had in deterministic case.
\newpage
\subsection{Convergence analysis for the strongly convex semi-stochastic case}
Before stating the convergence results for the strongly convex case, let us mention the following lemma  
\begin{lemma}\label{lemma:Dinh's strong}
	(Lemma 15 of \cite{blah}) Given \( \mu_f \geq 0 \), \( L_k \geq \mu_f \), and \( \tau_{k} \in (0,1) \), let \( m_k := \tfrac{L_k}{L_{k-1}} \) and \( \{x_k\}\) be a given sequence in \( \mathbb{R}^k \). We define \( \hat{x}_k := x_k + \beta_k \left( x_k - x_{k-1} \right) \), where \( \beta_k := \tfrac{(1 - \tau_{k-1})\tau_{k-1}}{\tau_{k-1}^2+m_k\tau_{k}} \).
	
	Assume that the following two conditions hold:
	\[
	L_{k-1} (1-\tau_{k})\tau_{k-1}^2 + \mu_f(1-\tau_{k})\tau_{k} \geq (L_k-\mu_f)\tau_{k}^2
	\]
	\[
L_{k-1} (\tau_{k-1}^2+ m_k\tau_{k})m_k\tau_{k}\geq (L_k-\mu_f)\tau_{k-1}^2
	\]
	
	Then, for any \( x \in \mathbb{R}^k \), we have
	\[
	(L_k-\mu_f)\tau_{k}^2\gnorm{\tfrac{1}{\tau_{k}}[\hat{x}_k-(1-\tau_{k})x_k]-x}{}{2} - \mu_f\tau_{k}(1-\tau_{k})\gnorm{x_k-x}{}{2}\leq 	L_{k-1} (1-\tau_{k})\tau_{k-1}^2\gnorm{\tfrac{1}{\tau_{k-1}}[x_k-(1-\tau_{k-1})x_{k-1}]-x}{}{2}. 
	\]
	
\end{lemma}
\begin{theorem}\label{thm:non-ergo-strong-semi}
	Suppose $\mu_f>0$ and we have the following step-size policy for $\{\tau_{k},\rho_{k},\eta_k,\beta_{k+1}\}_{k\geq 1}$
	\begin{equation}\label{eq:non-ergo-stepsize-strong}
		\begin{aligned}
			&\tau_{k+1} = \tfrac{\tau_k}{2}(\sqrt{\tau_k^2+4}-\tau_k), \quad \rho_{k+1} = \tfrac{\rho_1}{\tau_{k+1}^2},\quad
			\eta_k = \rho_k,\quad \beta_{k+1} = \tfrac{(1-\tau_{k})\tau_{k} L_{k}}{\tau_{k}^2 L_{k} + L_{k+1}\tau_{k+1}}\\
			& L_k =2(L_f + B L_g+\rho_k (M_g + M_\chi)^2),
		\end{aligned}
	\end{equation}
	where $\tau_1 = 1$, $ \rho_{1}=\tfrac{\mu_f}{(M_g + M_\chi)^2}$. 
	Then we have the following expected optimality and feasibility gaps
	\begin{equation}\label{eq:opt-1-non-ergo}
		\begin{aligned}
					\Ebb[\psi_0(x_K) - \psi(x^*)]\leq& \tfrac{4}{(K+1)^2}[4(L_f+BL_g)D_X^2+ \tfrac{1}{2\eta_{1}}\|y_1\|^2 ]+ \tfrac{4(K+2)( H_f^2+\sigma^2)}{\mu_f(K+1)^2}
		\end{aligned}
	\end{equation}
	\begin{equation}\label{eq:feasib-1-non-ergo}
		\begin{aligned}
					\Ebb[\|[\psi(x_K)]_+\|]&\leq \tfrac{4}{(K+1)^2}[(L_f+BL_g)\|x_1-x^*\|^2
				 + \tfrac{1}{2\eta_{1}}\|y_1-\hat{y}\|^2]+ \tfrac{(16K+9)[\mathcal{H}_*^2 +8( H_f^2+\sigma^2)]}{8\mu_f(K+1)^2},
		\end{aligned}
	\end{equation}
	where $\hat{y} = (\|y^*\|+1)\tfrac{[g(\bar{x}_K)]_+}{\|[g(\bar{x}_K)]_+\|}$ and $\mathcal{H}_* = (L_gD_x[\|y^*\|+1-B]_++ H_g(\|y^*\|+1))$.
\end{theorem}
\begin{proof}
	First of all, the updates in \eqref{eq:non-ergo-stepsize-strong} leads to the following equations for all $k\geq 2$
	\begin{equation*}\label{eq:relations-last-iter}
		\tau_k^2 = (1-\tau_k)\tau_{k-1}^2, \quad \tfrac{1}{k}\leq \tau_{k-1}\leq\tfrac{2}{k+1}.
	\end{equation*}
	Thus, $\rho_{k-1} = \tfrac{\rho_{1}}{\tau_{k-1}^2} = \tfrac{(1-\tau_k)\rho_1}{\tau_k^2} = (1-\tau_k)\rho_k$ which together with $\eta_k = \rho_{k}$ implies 
	\begin{equation*}\label{eq:relations-last-iter-2}
		 \eta_k<2\rho_k , \quad \tfrac{1}{\eta_k}= \tfrac{1-\tau_k}{\eta_{k-1}}, \quad \forall k\geq 2.
	\end{equation*}
	In addition, since $0< \rho_1=\tfrac{\mu_f}{(M_g + M_\chi)^2}$, then the following condition holds 
	\begin{subequations}
		\begin{equation*}
			L_{k-1}(1-\tau_k)\tau_{k-1}^2 + \mu_f(1-\tau_k)\tau_k\geq(L_k-\mu_f)\tau_k^2
		\end{equation*}
		\begin{equation*}
			L_{k-1}(\tau_{k-1}^2 + m_k\tau_k)m_k\tau_k \geq(L_k-\mu_f)\tau_{k-1}^2, \quad \forall k\geq 2
		\end{equation*}
	\end{subequations}
	where $m_k = \tfrac{L_k}{L_{k-1}}$. Hence we have the following useful relation for any $x\in X$. 
	\begin{equation}\label{eq:resultlemma15}
		\begin{aligned}
			&(L_k-\mu_f)\tau_k^2\gnorm{\tfrac{1}{\tau_k}[\wh{x}_k-(1-\tau_k)x_k] -x}{}{2}-\mu_f(1-\tau_k)\tau_k\|x_k-x\|^2\\
			\leq &(1-\tau_k)L_{k-1}\tau_{k-1}^2\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}, \quad \forall k\geq 2,
		\end{aligned}
	\end{equation}
	Now, substituting \eqref{eq:resultlemma15} into Lemma \ref{lemma:importantlemma}, one can obtain the following result for all $k\geq 2$
	\begin{equation}\label{eq:recur1}
		\begin{aligned}
			\Lcal(x_{k+1}, s_{k+1}, y) -& \Lcal(x,s,\wb{y}_{k+1})  
			\le(1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)]\\
			&+\tfrac{(1-\tau_k)L_{k-1}\tau_{k-1}^2}{2}\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}\\
			&\quad - \tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}   + \tfrac{1-\tau_k}{2\eta_{k-1}}\gnorm{y-\wt{y}_k}{}{2} -\tfrac{1}{2\eta_k} \gnorm{y-\wt{y}_{k+1}}{}{2}\\
			&\quad  + \tfrac{(L_gD_x[\|y\|-B]_+ + H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}-\tau_k\inner{\delta_k }{\dot{x}_k-x}.
		\end{aligned}
	\end{equation}
	By rearranging \eqref{eq:recur1} we have the following result 
	\begin{equation}\label{eq:recur2}
		\begin{aligned}
			\Lcal(x_{k+1}, &s_{k+1}, y) - \Lcal(x,s,\wb{y}_{k+1})+\tfrac{L_k\tau_k^2}{2}\gnorm{\tfrac{1}{\tau_k}[x_{k+1} - (1-\tau_k)x_k] - x}{}{2}+ \tfrac{1}{2\eta_k} \gnorm{y-\wt{y}_{k+1}}{}{2}  \\
			&\le(1-\tau_k)[\Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)+\tfrac{L_{k-1}\tau_{k-1}^2}{2}\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}\\
			&\quad + \tfrac{1}{2\eta_{k-1}}\gnorm{y-\wt{y}_k}{}{2} ] -\tau_{k}\inner{\delta_k }{\dot{x}_k-x} + \tfrac{(L_gD_x[\|y\|-B]_+ + H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k} .
		\end{aligned}
	\end{equation}
	Let us consider $Q_k(x,y)$ s follows 
	\[
	Q_k(x,y)  = \Lcal(x_k, s_k, y) - \Lcal(x,s,\wb{y}_k)+\tfrac{L_{k-1}\tau_{k-1}^2}{2}\gnorm{\tfrac{1}{\tau_{k-1}}[x_{k} - (1-\tau_{k-1})x_{k-1}] - x}{}{2}+ \tfrac{1}{2\eta_{k-1}}\gnorm{y-\wt{y}_k}{}{2}.
	\]
	Hence \eqref{eq:recur2} implies the following 
	\begin{equation}\label{eq:Q_recur}
			Q_{k+1}(x,y)\leq (1-\tau_k)Q_k(x,y)  +  \tau_{k}\inner{\delta_k }{x-\dot{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}, \quad \forall k\geq 2.
	\end{equation}
Moreover regarding  initialization in Algorithm \ref{alg:augConEx}, Lemma \ref{lemma:importantlemma} and the step-size policy in Theorem \ref{thm:non-ergo-strong-semi}, we have the following relations for $k=2$ 
\begin{equation}\label{eq:Q_1}
	Q_2(x,y)\leq \tfrac{L_1-\mu_f}{2}\|x_1-x\|^2 + \tfrac{1}{2\eta_{1}}\|y_1-y\|^2+ \tfrac{(L_gD_x[\|y\|-B]_+ + H_g\|y\|)^2}{4(L_1-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_1\|^2)}{L_1}-\inner{\delta_1 }{\dot{x}_1-x}.
\end{equation}
	Using the recursion in \eqref{eq:Q_recur} from $k=2$ to $K-1$ and considering $\tau_1 =1, \tilde{y}_1 = y_1$, and $ \hat{x}_1 = x_1$ we have 
	\begin{equation}\label{eq:recur3}
		\begin{aligned}
			\Lcal(x_{K}, &s_{K}, y) - \Lcal(x,s,\wb{y}_{K}) 
			\le[\prod_{k=2}^{K-1} (1-\tau_{k})]Q_2(x,y)
			\\
			&\quad +\sum_{k=2}^{K-1}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})]\tau_{k} \inner{\delta_k }{x-\dot{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big]\\
			&\leq \tfrac{4}{(K+1)^2}[(L_f+BL_g)\|x_1-x\|^2+ \tfrac{1}{2\eta_{1}}\|y_1-y\|^2 + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4\rho_{1}(M_g+M_\chi)^2}\\
			&\quad+\tfrac{H_f^2+\|\delta_1\|^2}{(L_f+BL_g+\rho_{1}(M_g + M_\chi^2))} - \inner{\delta_1}{\dot{x}_1-x}] +\inner{\delta_{K-1}}{x-\hat{x}_{K-1}} + \tfrac{(L_gD_x  [\| y\| - B]_++H_g\|y\|)^2}{4(L_{K-1}-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \|\delta_{K-1}\|^2)}{L_{K-1}}\\
			&\quad	 +\sum_{k=2}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tau_{k}\inner{\delta_k }{x-\hat{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big],
		\end{aligned}
	\end{equation}
	where we used \eqref{eq:Q_1}, $\rho_{1}(M_g+M_{\chi})^2= \mu_f$  and $[\prod_{k=2}^{K-1} (1-\tau_{k})] = \tfrac{\tau_{K-1}^2}{\tau_1}\leq \tfrac{4}{(K+1)^2}$ to obtain the second inequality. 	
	We know that $ \Lcal(x_K,y)\leq \Lcal(x_K,s_K,y)$ and for $s =0 $, we have $\Lcal(x,\bar{y}_K) = \Lcal(x,0,\bar{y}_K)$ leading to the following relation 
	\begin{equation}\label{eq:relation3}
		\Lcal(x_K,y) - \Lcal(x,\bar{y}_K) \leq \Lcal(x_K,s_K,y) - \Lcal(x,0,\bar{y}_K).
	\end{equation}
	Using \eqref{eq:relation3}, with \eqref{eq:recur3} alongside definition of $  \Lcal(x,y)$ we have 
	\begin{equation}\label{eq:non-ergo-8}
		\begin{aligned}
			&\psi_0(x_K)+ \langle y , \psi(x_K)\rangle - \psi_0(x) - \langle \bar{y}_K, \psi(x)\rangle \leq  \tfrac{4}{(K+1)^2}[(L_f+BL_g)\|x_1-x\|^2\\
			 &\quad+ \tfrac{1}{2\eta_{1}}\|y_1-y\|^2+\tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2 +4(H_f^2+\|\delta_1\|^2)}{4\rho_{1}(M_g+M_\chi)^2)}- \inner{\delta_1}{\dot{x}_1-x}]
			 \\&\quad +\sum_{k=2}^{K-1}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \tau_{k}\inner{\delta_k }{x-\dot{x}_k} + \tfrac{(L_gD_x[\|y\|-B]_++H_g\|y\|)^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big]
		\end{aligned}
	\end{equation}
	Now let us choose $ y =0 $. we know $ \bar{y}_K\geq 0$ and $\psi(x^*)\leq 0$, thus $ \langle \bar{y}_K, \psi(x^\ast)\rangle \leq 0 $. Rewriting \eqref{eq:non-ergo-8} for $(x,y)=(x^*,0)$ and taking the expectation from both sides with respect to $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0 $, one can conclude the following 
	\begin{equation}\label{eq:feasib}
		\begin{aligned}
				\Ebb[\psi_0(x_K) - \psi(x^*)]\leq& \tfrac{4}{(K+1)^2}[(L_f+BL_g)4D_X^2
				+ \tfrac{1}{2\eta_{1}}\|y_1\|^2 + \tfrac{(H_f^2+\sigma^2)}{\rho_{1}(M_g+M_\chi)^2} ]\\
				&\quad	+\sum_{k=2}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})]  \tfrac{2(H_f^2+\sigma^2)}{L_k}\big] + \tfrac{H_f^2+ \sigma^2}{\rho_{K-1}(M_g+M_\chi)^2}.
		\end{aligned}
	\end{equation}
	Now let us focus on the following summation 
	\begin{equation}\label{eq:first-sum}
		\begin{aligned}
			 \sum_{k=2}^{K-2} [\prod_{i=k+1}^{K-1} (1-\tau_{i})]\tfrac{2(H_f^2+\sigma^2)}{L_k}
			&\leq \sum_{k=2}^{K-2} \tfrac{\tau_{K-1}^2}{\tau_{k}^2}\tfrac{H_f^2+\sigma^2}{\rho_k (M_g+M_\chi)^2} \leq \tfrac{4(H_f^2+\sigma^2)}{(K+1)^2}\sum_{k=2}^{K-2} \tfrac{1}{\rho_1 (M_g+M_\chi)^2} \leq\tfrac{4K(H_f^2+\sigma^2)}{(K+1)^2\mu_f},
		\end{aligned}
	\end{equation}
	where we used $\tfrac{1}{k+1}\leq \tau_k\leq\tfrac{2}{k+2}$ and $\rho_{1}(M_g+M_\chi)^2=\mu_f$ in the last two inequalities. Moreover, note that $\tfrac{H_f^2+ \sigma^2}{\rho_{K-1}(M_g+M_\chi)^2} = \tfrac{4(H_f^2+\sigma^2)}{(K+1)^2\mu_f}$.Therefore, using \eqref{eq:feasib} and \eqref{eq:first-sum}, we concludes \eqref{eq:opt-1-non-ergo}.
	 Now let us focus on the feasibility convergence rate. First, we rewrite \eqref{eq:non-ergo-8} for any $ x=x^*$ and $\hat{y}$, where $\hat{y} = (\|y^*\|+1)\tfrac{[g(\bar{x}_K)]_+}{\|[g(\bar{x}_K)]_+\|}$.  We have 
	\begin{equation}\label{eq:non-ergo-10}
		\begin{aligned}
			\psi&_0(x_K)+ \langle \hat{y} , \psi(x_K)\rangle - \psi_0(x^*) - \langle \bar{y}_K, \psi(x^*)\rangle \leq  \tfrac{4}{(K+1)^2}[(L_f+BL_g) \|x_1-x^*\|^2\\
			&+ \tfrac{1}{2\eta_{1}}\|y_1-\hat{y}\|^2+\tfrac{\mathcal{H}_*^2 +4(H_f^2+\|\delta_1\|^2)}{4\rho_{1}(M_g+M_\chi)^2} - \inner{\delta_1}{\dot{x}_1-x^*}]+ \big[\tfrac{\mathcal{H}_*^2}{4(L_{K-1}-2(L_f+ BL_g ))}+\inner{\delta_{K-1}}{x^*-\dot{x}_{K-1}}  + \tfrac{2(H_f^2+ \|\delta_k\|^2)}{L_{K-1}}\big]\\
			&\quad
			+\sum_{k=1}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \inner{\delta_k }{x^*-\hat{x}_k} + \tfrac{\mathcal{H}_*^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big]\\
			&.
		\end{aligned}
	\end{equation}
	Using the similar argument in Theorem \ref{thm:convex-case}, one can conclude the following
	\begin{equation}\label{eq:non-ergo-feas-10}
		\begin{aligned}
			\|[ \psi({x}_K)]_+\|& \leq  \tfrac{4}{(K+1)^2}[(L_f+BL_g)\|x_1-x^*\|+ \tfrac{1}{2\eta_{1}}\|y_1-\hat{y}\|^2 
			+ \tfrac{\mathcal{H}_*^2 + 4(H_f^2+\|\delta_k\|^2)}{4\rho_{1}(M_g+M_\chi)^2}+ \inner{\delta_1}{x-\dot{x}_1}]\\
			&\quad+\inner{\delta_{K-1}}{x-\hat{x}_{K-1}}+\big[\tfrac{\mathcal{H}_*^2}{4(L_{K-1}-2(L_f+ BL_g ))} + \tfrac{2(H_f^2+ \|\delta_{K-1}\|^2)}{L_{K-1}}\big]\\
			&\quad+\sum_{k=1}^{K-2}\big[ [\prod_{i=k+1}^{K-1} (1-\tau_{i})] \inner{\delta_k }{x-\hat{x}_k} + \tfrac{\mathcal{H}_*^2}{4(L_k-2(L_f + BL_g))}+ \tfrac{2(H_f^2+\|\delta_k\|^2)}{L_k}\big].
		\end{aligned}
	\end{equation} 
	Taking the expectation from both sides of \eqref{eq:non-ergo-feas-10} with respect to $\Ebb[\inner{\delta_k}{\dot{x}_k-x^*}] = 0 $, using similar relations we had in \eqref{eq:first-sum}, and $\rho_{1}(M_g+M_\chi)^2= \mu_f$ one concludes \eqref{eq:feasib-1-non-ergo}. 
	
\end{proof}
Similar to Theorem \ref{thm:convex-case}, Theorem \ref{thm:non-ergo-strong-semi} provides the convergence rate of error for the stochastic non-smooth function constrained optimization problem with strong convexity assumption. In general \aconex obtain the following convergence rate for the strongly-convex problem with modulus $\mu_f$ 
\[
\mathcal{O}\big( \tfrac{D_X^2(L_f+BL_g)}{K^2} + \tfrac{\mathcal{H}_*^2+H_f^2+\sigma^2}{\mu_fK}\big)
\] 
Notice the overall convergence rate is of order $\mathcal{O}(\tfrac{1}{\rho_{1}K})$ meaning that choosing an extremely small value for $\rho_{1}$ will lead to divergence. Specifically, $\rho_{1}$ should be in order of $\Omega(K^{-1})$.
Note that unlike the step-size policy in the convex case, $L_k$ is increasing with respect to $\rho_k$ in each iteration. In particular, one can observe that the change rate in $L_k$ is of order $\mathcal{O}(k^2)$. 

